Computing Scaled Relative Graphs of Discrete-time LTI Systems from Data

Graphical methods for system analysis have played a central role in control theory. The Scaled Relative Graph (SRG) has recently emerged as a useful tool for stability analysis of feedback interconnections. In this paper, we further extend its applicability by showing how the SRG of a discrete-time linear-time-invariant (LTI) system can be computed exactly from its state-space representation using linear matrix inequalities. We additionally propose a fully data-driven approach where we demonstrate how to compute the SRG exclusively from input-output data. Furthermore, we introduce a robust version of the SRG, which can be computed from noisy data trajectories and contains the SRG of the actual system.

==> data/SRG/robust_MIMO_unstable.tex <==
\draw[fill=DutchBlue!80](0.0473, 0.0031) to (0.0475, 0.0000) to (0.0468, 0.0000) to (0.0484, 0.0000) to (0.0500, 0.0000) to (0.0515, 0.0000) to (0.0531, 0.0000) to (0.0547, 0.0000) to (0.0563, 0.0000) to (0.0583, 0.0000) to (0.0598, 0.0000) to (0.0614, 0.0000) to (0.0630, 0.0000) to (0.0646, 0.0000) to (0.0662, 0.0000) to (0.0677, 0.0000) to (0.0693, 0.0000) to (0.0709, 0.0000) to (0.0725, 0.0000) to (0.0741, 0.0000) to (0.0757, 0.0000) to (0.0773, 0.0000) to (0.0788, 0.0000) to (0.0804, 0.0000) to (0.0820, 0.0000) to (0.0836, 0.0000) to (0.0852, 0.0000) to (0.0867, 0.0000) to (0.0883, 0.0000) to (0.0899, 0.0000) to (0.0915, 0.0000) to (0.0931, 0.0000) to (0.0947, 0.0000) to (0.0962, 0.0000) to (0.0978, 0.0000) to (0.0994, 0.0000) to (0.1010, 0.0000) to (0.1026, 0.0000) to (0.1042, 0.0000) to (0.1058, 0.0000) to (0.1074, 0.0000) to (0.1089, 0.0000) to (0.1105, 0.0000) to (0.1121, 0.0000) to (0.1137, 0.0000) to (0.1153, 0.0000) to (0.1169, 0.0000) to (0.1185, 0.0000) to (0.1201, 0.0000) to (0.1218, 0.0000) to (0.1234, 0.0000) to (0.1250, 0.0000) to (0.1266, 0.0000) to (0.1282, 0.0000) to (0.1298, 0.0000) to (0.1314, 0.0000) to (0.1330, 0.0000) to (0.1346, 0.0000) to (0.1362, 0.0000) to (0.1378, 0.0000) to (0.1394, 0.0000) to (0.1410, 0.0000) to (0.1426, 0.0000) to (0.1442, 0.0000) to (0.1458, 0.0000) to (0.1474, 0.0000) to (0.1490, 0.0000) to (0.1506, 0.0000) to (0.1522, 0.0000) to (0.1544, 0.0000) to (0.1561, 0.0000) to (0.1577, 0.0000) to (0.1593, 0.0000) to (0.1609, 0.0000) to (0.1625, 0.0000) to (0.1641, 0.0000) to (0.1657, 0.0000) to (0.1673, 0.0000) to (0.1689, 0.0000) to (0.1706, 0.0000) to (0.1722, 0.0000) to (0.1738, 0.0000) to (0.1754, 0.0000) to (0.1770, 0.0000) to (0.1787, 0.0000) to (0.1803, 0.0000) to (0.1819, 0.0000) to (0.1835, 0.0000) to (0.1852, 0.0000) to (0.1868, 0.0000) to (0.1884, 0.0000) to (0.1900, 0.0000) to (0.1917, 0.0000) to (0.1933, 0.0000) to (0.1949, 0.0000) to (0.1965, 0.0000) to (0.1982, 0.0000) to (0.1998, 0.0000) to (0.2014, 0.0000) to (0.2031, 0.0000) to (0.2047, 0.0000) to (0.2064, 0.0000) to (0.2080, 0.0000) to (0.2096, 0.0000) to (0.2113, 0.0000) to (0.2129, 0.0000) to (0.2146, 0.0000) to (0.2162, 0.0000) to (0.2178, 0.0000) to (0.2195, 0.0000) to (0.2211, 0.0000) to (0.2228, 0.0000) to (0.2244, 0.0000) to (0.2261, 0.0000) to (0.2277, 0.0000) to (0.2294, 0.0000) to (0.2310, 0.0000) to (0.2327, 0.0000) to (0.2344, 0.0000) to (0.2360, 0.0000) to (0.2377, 0.0000) to (0.2393, 0.0000) to (0.2410, 0.0000) to (0.2427, 0.0000) to (0.2443, 0.0000) to (0.2460, 0.0000) to (0.2477, 0.0000) to (0.2493, 0.0000) to (0.2510, 0.0000) to (0.2527, 0.0000) to (0.2543, 0.0000) to (0.2560, 0.0000) to (0.2577, 0.0000) to (0.2594, 0.0000) to (0.2610, 0.0000) to (0.2627, 0.0000) to (0.2644, 0.0000) to (0.2661, 0.0000) to (0.2678, 0.0000) to (0.2705, 0.0000) to (0.2722, 0.0000) to (0.2738, 0.0000) to (0.2755, 0.0000) to (0.2772, 0.0000) to (0.2789, 0.0000) to (0.2806, 0.0000) to (0.2823, 0.0000) to (0.2840, 0.0000) to (0.2857, 0.0000) to (0.2874, 0.0000) to (0.2891, 0.0000) to (0.2908, 0.0000) to (0.2925, 0.0000) to (0.2942, 0.0000) to (0.2959, 0.0000) to (0.2976, 0.0000) to (0.2993, 0.0000) to (0.3011, 0.0000) to (0.3028, 0.0000) to (0.3045, 0.0000) to (0.3062, 0.0000) to (0.3080, 0.0000) to (0.3097, 0.0000) to (0.3114, 0.0000) to (0.3131, 0.0000) to (0.3149, 0.0000) to (0.3166, 0.0000) to (0.3183, 0.0000) to (0.3200, 0.0000) to (0.3256, 0.0112) to (0.3299, 0.0194) to (0.3343, 0.0273) to (0.3536, 0.0513) to (0.4149, 0.0769) to (0.4541, 0.0744) to (0.4818, 0.0668) to (0.5041, 0.0577) to (0.5232, 0.0482) to (0.5405, 0.0381) to (0.5562, 0.0279) to (0.5711, 0.0170) to (0.5852, 0.0015) to (0.5932, 0.0000) to (0.5954, 0.0000) to (0.5975, 0.0000) to (0.5996, 0.0000) to (0.6018, 0.0000) to (0.6039, 0.0000) to (0.6060, 0.0000) to (0.6082, 0.0000) to (0.6116, 0.0000) to (0.6138, 0.0000) to (0.6159, 0.0000) to (0.6181, 0.0000) to (0.6203, 0.0000) to (0.6224, 0.0000) to (0.6246, 0.0000) to (0.6268, 0.0000) to (0.6290, 0.0000) to (0.6312, 0.0000) to (0.6334, 0.0000) to (0.6356, 0.0000) to (0.6378, 0.0000) to (0.6400, 0.0000) to (0.6422, 0.0000) to (0.6444, 0.0000) to (0.6467, 0.0000) to (0.6489, 0.0000) to (0.6511, 0.0000) to (0.6534, 0.0000) to (0.6560, 0.0000) to (0.6582, 0.0000) to (0.6605, 0.0000) to (0.6627, 0.0000) to (0.6650, 0.0000) to (0.6673, 0.0000) to (0.6695, 0.0000) to (0.6718, 0.0000) to (0.6741, 0.0000) to (0.6764, 0.0000) to (0.6781, 0.0000) to (0.6804, 0.0000) to (0.6827, 0.0000) to (0.6850, 0.0000) to (0.6873, 0.0000) to (0.6896, 0.0000) to (0.6919, 0.0000) to (0.6943, 0.0000) to (0.6966, 0.0000) to (0.6989, 0.0000) to (0.7013, 0.0000) to (0.7036, 0.0000) to (0.7060, 0.0000) to (0.7083, 0.0000) to (0.7107, 0.0000) to (0.7130, 0.0000) to (0.7154, 0.0000) to (0.7178, 0.0000) to (0.7202, 0.0000) to (0.7226, 0.0000) to (0.7250, 0.0000) to (0.7274, 0.0000) to (0.7298, 0.0000) to (0.7322, 0.0000) to (0.7346, 0.0000) to (0.7370, 0.0000) to (0.7394, 0.0000) to (0.7419, 0.0000) to (0.7443, 0.0000) to (0.7468, 0.0000) to (0.7492, 0.0000) to (0.7517, 0.0000) to (0.7541, 0.0000) to (0.7566, 0.0000) to (0.7658, 0.0137) to (0.7742, 0.0264) to (0.7825, 0.0385) to (0.7903, 0.0503) to (0.7978, 0.0619) to (0.8051, 0.0734) to (0.8119, 0.0846) to (0.8185, 0.0958) to (0.8226, 0.1032) to (0.8263, 0.1098) to (0.8293, 0.1154) to (0.8324, 0.1209) to (0.8355, 0.1270) to (0.8382, 0.1321) to (0.8413, 0.1382) to (0.8438, 0.1433) to (0.8466, 0.1490) to (0.8490, 0.1540) to (0.8515, 0.1593) to (0.8686, 0.1925) to (1.3106, 0.3934) to (1.5205, 0.2856) to (1.5326, 0.2742) to (1.5451, 0.2623) to (1.5568, 0.2510) to (1.5694, 0.2387) to (1.5808, 0.2276) to (1.5934, 0.2147) to (1.6045, 0.2039) to (1.6173, 0.1903) to (1.6280, 0.1798) to (1.6386, 0.1682) to (1.6513, 0.1554) to (1.6614, 0.1442) to (1.6744, 0.1305) to (1.6842, 0.1199) to (1.6974, 0.1049) to (1.7069, 0.0951) to (1.7172, 0.0825) to (1.7293, 0.0697) to (1.7383, 0.0589) to (1.7517, 0.0427) to (1.7603, 0.0339) to (1.7702, 0.0181) to (1.7822, 0.0055) to (1.7870, 0.0000) to (1.7936, 0.0000) to (1.8002, 0.0000) to (1.8040, 0.0000) to (1.8107, 0.0000) to (1.8175, 0.0000) to (1.8242, 0.0000) to (1.8311, 0.0000) to (1.8379, 0.0000) to (1.8442, 0.0000) to (1.8493, 0.0000) to (1.8563, 0.0000) to (1.8633, 0.0000) to (1.8703, 0.0000) to (1.8774, 0.0000) to (1.8844, 0.0000) to (1.8916, 0.0000) to (1.8988, 0.0000) to (1.9061, 0.0000) to (1.9134, 0.0000) to (1.9207, 0.0000) to (1.9213, 0.0000) to (1.9246, 0.0000) to (1.9320, 0.0000) to (1.9395, 0.0000) to (1.9470, 0.0000) to (1.9545, 0.0000) to (1.9621, 0.0000) to (1.9648, 0.0000) to (1.9725, 0.0000) to (1.9802, 0.0000) to (1.9879, 0.0000) to (1.9957, 0.0000) to (1.9979, 0.0000) to (2.0050, 0.0000) to (2.0129, 0.0000) to (2.0209, 0.0000) to (2.0289, 0.0000) to (2.0370, 0.0000) to (2.0451, 0.0000) to (2.0452, 0.0000) to (2.0534, 0.0000) to (2.0616, 0.0000) to (2.0699, 0.0000) to (2.0782, 0.0000) to (2.0794, 0.0000) to (2.0854, 0.0000) to (2.0939, 0.0000) to (2.1023, 0.0000) to (2.1109, 0.0000) to (2.1195, 0.0000) to (2.1256, 0.0000) to (2.1343, 0.0000) to (2.1431, 0.0000) to (2.1519, 0.0000) to (2.1608, 0.0000) to (2.1658, 0.0000) to (2.1665, 0.0000) to (2.1754, 0.0000) to (2.1951, 0.0228) to (2.2061, 0.0391) to (2.2142, 0.0483) to (2.2274, 0.0638) to (2.2416, 0.0818) to (2.2493, 0.0919) to (2.2581, 0.1022) to (2.2729, 0.1209) to (2.2838, 0.1353) to (2.2909, 0.1445) to (2.3013, 0.1576) to (2.3150, 0.1756) to (2.3245, 0.1886) to (2.3310, 0.1973) to (2.3413, 0.2110) to (2.3540, 0.2283) to (2.3637, 0.2419) to (2.3698, 0.2505) to (2.3784, 0.2624) to (2.3902, 0.2791) to (2.4016, 0.2956) to (2.4073, 0.3039) to (2.4128, 0.3119) to (2.4238, 0.3280) to (2.4344, 0.3438) to (2.4495, 0.3663) to (2.4661, 0.3901) to (2.4884, 0.4194) to (2.5271, 0.4669) to (2.5705, 0.5147) to (2.6163, 0.5605) to (2.6427, 0.5852) to (2.6748, 0.6126) to (2.7383, 0.6629) to (2.8118, 0.7138) to (2.8975, 0.7644) to (2.9685, 0.8006) to (3.0232, 0.8244) to (3.1183, 0.8584) to (3.2621, 0.8948) to (3.4362, 0.9147) to (3.6487, 0.9030) to (3.8420, 0.8562) to (3.9872, 0.7927) to (4.1934, 0.6442) to (4.2652, 0.5714) to (4.2932, 0.5399) to (4.3194, 0.5092) to (4.3441, 0.4794) to (4.3584, 0.4618) to (4.3698, 0.4473) to (4.3892, 0.4220) to (4.4098, 0.3945) to (4.4292, 0.3678) to (4.4475, 0.3418) to (4.4616, 0.3214) to (4.4699, 0.3091) to (4.4761, 0.2999) to (4.4810, 0.2924) to (4.4859, 0.2850) to (4.4898, 0.2789) to (4.4965, 0.2683) to (4.5029, 0.2584) to (4.5083, 0.2497) to (4.5153, 0.2384) to (4.5205, 0.2300) to (4.5271, 0.2190) to (4.5321, 0.2109) to (4.5378, 0.2010) to (4.5431, 0.1922) to (4.5477, 0.1842) to (4.5536, 0.1739) to (4.5580, 0.1662) to (4.5636, 0.1561) to (4.5678, 0.1488) to (4.5727, 0.1398) to (4.5767, 0.1327) to (4.5772, 0.1317) to (4.5811, 0.1243) to (4.5861, 0.1150) to (4.5899, 0.1080) to (4.5947, 0.0988) to (4.5982, 0.0921) to (4.6025, 0.0834) to (4.6063, 0.0765) to (4.6096, 0.0696) to (4.6139, 0.0612) to (4.6171, 0.0547) to (4.6212, 0.0462) to (4.6243, 0.0402) to (4.6280, 0.0318) to (4.6312, 0.0259) to (4.6340, 0.0190) to (4.6378, 0.0117) to (4.6405, 0.0047) to (4.6426, 0.0000) to (4.6583, 0.0000) to (4.6667, 0.0000) to (4.6684, 0.0000) to (4.6750, 0.0) to (4.685, 0.0) to (4.6970, 0.0000) to (4.6985, 0.0000) to (4.7050, 0.0) to (4.7150, 0.0) to (4.7273, 0.0000) to (4.7300, 0.0) to (4.7387, 0.0000) to (4.74, 0.0) to (4.75, 0.0) to (4.7576, 0.0000) to (4.76, 0.0) to (4.77, 0.0) to (4.7789, 0.0000) to (4.7879, 0.0000) to (4.795, 0.0) to (4.805, 0.0) to (4.81,0.0) to (4.8182, 0.0000) to (4.8191,0.0000)
to (4.8291,0.0000)
to (4.8391,0.0000)
to (4.8485,0.0000)
to (4.8585,0.0000)
to (4.8593,0.0000)
to (4.8693,0.0000)
to (4.8788,0.0000)
to (4.8888,0.0000)
to (4.8988,0.0000)
to (4.8995,0.0000)
to (4.9091,0.0000)
to (4.9191,0.0000)
to (4.9291,0.0000)
to (4.9391,0.0000)
to (4.9394,0.0000)
to (4.9397,0.0000)
to (4.9497,0.0000)
to (4.9597,0.0000)
to (4.9697,0.0000)
to (4.9797,0.0000)
to (4.9799,0.0000)
to (4.9899,0.0000)
to (4.9999,0.0000)
to (5.0000,0.0000)
to (5.0100,0.0000)
to (5.0200,0.0000)
to (5.0201,0.0000)
to (5.0301,0.0000)
to (5.0303,0.0000)
to (5.0403,0.0000)
to (5.0503,0.0000)
to (5.0577,0.0000)
to (5.0603,0.0000)
to (5.0606,0.0000)
to (5.0706,0.0000)
to (5.0806,0.0000)
to (5.0906,0.0000)
to (5.0909,0.0000)
to (5.1005,0.0000)
to (5.1105,0.0000)
to (5.1205,0.0000)
to (5.1212,0.0000)
to (5.1312,0.0000)
to (5.1407,0.0000)
to (5.1507,0.0000)
to (5.1515,0.0000)
to (5.1615,0.0000)
to (5.1715,0.0000)
to (5.1809,0.0000)
to (5.1818,0.0000)
to (5.1918,0.0000)
to (5.2018,0.0000)
to (5.2118,0.0000)
to (5.2121,0.0000)
to (5.2211,0.0000)
to (5.2311,0.0000)
to (5.2411,0.0000)
to (5.2424,0.0000)
to (5.2524,0.0000)
to (5.2613,0.0000)
to (5.2713,0.0000)
to (5.2727,0.0000)
to (5.2827,0.0000)
to (5.2927,0.0000)
to (5.3015,0.0000)
to (5.3030,0.0000)
to (5.3130,0.0000)
to (5.3230,0.0000)
to (5.3330,0.0000)
to (5.3333,0.0000)
to (5.3417,0.0000)
to (5.3517,0.0000)
to (5.3617,0.0000)
to (5.3636,0.0000)
to (5.3736,0.0000)
to (5.3819,0.0000)
to (5.3919,0.0000)
to (5.3939,0.0000)
to (5.4039,0.0000)
to (5.4139,0.0000)
to (5.4221,0.0000)
to (5.4242,0.0000)
to (5.4342,0.0000)
to (5.4442,0.0000)
to (5.4542,0.0000)
to (5.4545,0.0000)
to (5.4623,0.0000)
to (5.4723,0.0000)
to (5.4823,0.0000)
to (5.4848,0.0000)
to (5.4948,0.0000)
to (5.5025,0.0000)
to (5.5125,0.0000)
to (5.5147,0.0000)
to (5.5152,0.0000)
to (5.5252,0.0000)
to (5.5352,0.0000)
to (5.5427,0.0000)
to (5.5455,0.0000)
to (5.5555,0.0000)
to (5.5655,0.0000)
to (5.5755,0.0000)
to (5.5758,0.0000)
to (5.5829,0.0000)
to (5.5929,0.0000)
to (5.6029,0.0000)
to (5.6061,0.0000)
to (5.6161,0.0000)
to (5.6231,0.0000)
to (5.6331,0.0000)
to (5.6364,0.0000)
to (5.6464,0.0000)
to (5.6564,0.0000)
to (5.6633,0.0000)
to (5.6667,0.0000)
to (5.6767,0.0000)
to (5.6867,0.0000)
to (5.6967,0.0000)
to (5.6970,0.0000)
to (5.7035,0.0000)
to (5.7135,0.0000)
to (5.7235,0.0000)
to (5.7273,0.0000)
to (5.7373,0.0000)
to (5.7437,0.0000)
to (5.7537,0.0000)
to (5.7576,0.0000)
to (5.7676,0.0000)
to (5.7776,0.0000)
to (5.7839,0.0000)
to (5.7879,0.0000)
to (5.7979,0.0000)
to (5.8079,0.0000)
to (5.8179,0.0000)
to (5.8182,0.0000)
to (5.8241,0.0000)
to (5.8341,0.0000)
to (5.8441,0.0000)
to (5.8485,0.0000)
to (5.8585,0.0000)
to (5.8643,0.0000)
to (5.8743,0.0000)
to (5.8788,0.0000)
to (5.8888,0.0000)
to (5.8988,0.0000)
to (5.9045,0.0000)
to (5.9091,0.0000)
to (5.9191,0.0000)
to (5.9291,0.0000)
to (5.9391,0.0000)
to (5.9394,0.0000)
to (5.9447,0.0000)
to (5.9547,0.0000)
to (5.9647,0.0000)
to (5.9697,0.0000)
to (5.9797,0.0000)
to (5.9849,0.0000)
to (5.9949,0.0000)
to (6.0000,0.0000)
to (6.0100,0.0000)
to (6.0200,0.0000)
to (6.0251,0.0000)
to (6.0303,0.0000)
to (6.0403,0.0000)
to (6.0503,0.0000)
to (6.0590,0.0000)
to (6.0606,0.0000)
to (6.0653,0.0000)
to (6.0753,0.0000)
to (6.0853,0.0000)
to (6.0909,0.0000)
to (6.1009,0.0000)
to (6.1055,0.0000)
to (6.1155,0.0000)
to (6.1212,0.0000)
to (6.1312,0.0000)
to (6.1412,0.0000)
to (6.1457,0.0000)
to (6.1515,0.0000)
to (6.1615,0.0000)
to (6.1715,0.0000)
to (6.1815,0.0000)
to (6.1818,0.0000)
to (6.1859,0.0000)
to (6.1959,0.0000)
to (6.2059,0.0000)
to (6.2121,0.0000)
to (6.2221,0.0000)
to (6.2261,0.0000)
to (6.2361,0.0000)
to (6.2424,0.0000)
to (6.2524,0.0000)
to (6.2624,0.0000)
to (6.2663,0.0000)
to (6.2727,0.0000)
to (6.2827,0.0000)
to (6.2927,0.0000)
to (6.3027,0.0000)
to (6.3030,0.0000)
to (6.3065,0.0000)
to (6.3165,0.0000)
to (6.3265,0.0000)
to (6.3333,0.0000)
to (6.3433,0.0000)
to (6.3467,0.0000)
to (6.3567,0.0000)
to (6.3636,0.0000)
to (6.3736,0.0000)
to (6.3836,0.0000)
to (6.3869,0.0000)
to (6.3939,0.0000)
to (6.4039,0.0000)
to (6.4139,0.0000)
to (6.4239,0.0000)
to (6.4242,0.0000)
to (6.4271,0.0000)
to (6.4371,0.0000)
to (6.4471,0.0000)
to (6.4545,0.0000)
to (6.4645,0.0000)
to (6.4673,0.0000)
to (6.4773,0.0000)
to (6.4848,0.0000)
to (6.4948,0.0000)
to (6.5048,0.0000)
to (6.5075,0.0000)
to (6.5152,0.0000)
to (6.5252,0.0000)
to (6.5352,0.0000)
to (6.5452,0.0000)
to (6.5455,0.0000)
to (6.5477,0.0000)
to (6.5577,0.0000)
to (6.5677,0.0000)
to (6.5758,0.0000)
to (6.5858,0.0000)
to (6.5879,0.0000)
to (6.5979,0.0000)
to (6.6061,0.0000)
to (6.6161,0.0000)
to (6.6261,0.0000)
to (6.6281,0.0000)
to (6.6364,0.0000)
to (6.6464,0.0000)
to (6.6564,0.0000)
to (6.6664,0.0000)
to (6.6667,0.0000)
to (6.6683,0.0000)
to (6.6783,0.0000)
to (6.6883,0.0000)
to (6.6970,0.0000)
to (6.7070,0.0000)
to (6.7085,0.0000)
to (6.7185,0.0000)
to (6.7187,0.0000)
to (6.7273,0.0000)
to (6.7373,0.0000)
to (6.7473,0.0000)
to (6.7487,0.0000) to (6.7563, 0.0012) to (6.7573, 0.0082) to (6.7582, 0.0110) to (6.7594, 0.0163) to (6.7603, 0.0198) to (6.7615, 0.0245) to (6.7624, 0.0281) to (6.7636, 0.0325) to (6.7644, 0.0362) to (6.7653, 0.0395) to (6.7664, 0.0441) to (6.7672, 0.0474) to (6.7683, 0.0518) to (6.7691, 0.0552) to (6.7702, 0.0594) to (6.7720, 0.0668) to (6.7740, 0.0752) to (6.7759, 0.0835) to (6.7778, 0.0916) to (6.7797, 0.0995) to (6.7815, 0.1073) to (6.7832, 0.1150) to (6.7849, 0.1225) to (6.7865, 0.1298) to (6.7881, 0.1371) to (6.7897, 0.1441) to (6.7912, 0.1511) to (6.7923, 0.1565) to (6.7931, 0.1599) to (6.7941, 0.1647) to (6.7955, 0.1713) to (6.7968, 0.1778) to (6.7982, 0.1842) to (6.7994, 0.1905) to (6.8007, 0.1967) to (6.8019, 0.2027) to (6.8031, 0.2087) to (6.8043, 0.2146) to (6.8054, 0.2204) to (6.8065, 0.2261) to (6.8076, 0.2317) to (6.8086, 0.2372) to (6.8097, 0.2426) to (6.8107, 0.2479) to (6.8116, 0.2532) to (6.8126, 0.2583) to (6.8135, 0.2634) to (6.8145, 0.2684) to (6.8153, 0.2734) to (6.8162, 0.2782) to (6.8171, 0.2830) to (6.8179, 0.2878) to (6.8187, 0.2924) to (6.8195, 0.2970) to (6.8200, 0.3001) to (6.8204, 0.3024) to (6.8210, 0.3060) to (6.8218, 0.3103) to (6.8225, 0.3147) to (6.8232, 0.3189) to (6.8239, 0.3231) to (6.8246, 0.3273) to (6.8253, 0.3314) to (6.8259, 0.3354) to (6.8266, 0.3394) to (6.8272, 0.3433) to (6.8337, 0.3821) to (6.8462, 0.4730) to (6.8568, 0.5730) to (6.8638, 0.6603) to (6.8683, 0.7373) to (6.8709, 0.8066) to (6.8726, 0.8875) to (6.8719, 0.9664) to (6.8709, 1.0122) to (6.8696, 1.0527) to (6.8679, 1.0898) to (6.8661, 1.1238) to (6.8641, 1.1552) to (6.8620, 1.1842) to (6.8599, 1.2111) to (6.8577, 1.2362) to (6.8555, 1.2596) to (6.8533, 1.2815) to (6.8513, 1.3003) to (6.8503, 1.3095) to (6.8501, 1.3112) to (6.8500, 1.3122) to (6.8499, 1.3134) to (6.8497, 1.3154) to (6.8494, 1.3174) to (6.8492, 1.3194) to (6.8490, 1.3214) to (6.8487, 1.3235) to (6.8485, 1.3256) to (6.8483, 1.3277) to (6.8480, 1.3297) to (6.8479, 1.3307) to (6.8478, 1.3319) to (6.8475, 1.3341) to (6.8473, 1.3361) to (6.8470, 1.3385) to (6.8467, 1.3407) to (6.8465, 1.3429) to (6.8462, 1.3452) to (6.8459, 1.3474) to (6.8458, 1.3486) to (6.8456, 1.3498) to (6.8453, 1.3522) to (6.8450, 1.3545) to (6.8447, 1.3571) to (6.8445, 1.3592) to (6.8441, 1.3618) to (6.8438, 1.3641) to (6.8437, 1.3654) to (6.8435, 1.3668) to (6.8432, 1.3693) to (6.8429, 1.3719) to (6.8425, 1.3745) to (6.8422, 1.3771) to (6.8418, 1.3797) to (6.8417, 1.3810) to (6.8415, 1.3824) to (6.8411, 1.3851) to (6.8408, 1.3879) to (6.8404, 1.3906) to (6.8400, 1.3934) to (6.8398, 1.3955) to (6.8396, 1.3969) to (6.8393, 1.3991) to (6.8389, 1.4020) to (6.8385, 1.4050) to (6.8380, 1.4079) to (6.8378, 1.4099) to (6.8376, 1.4114) to (6.8372, 1.4140) to (6.8368, 1.4171) to (6.8363, 1.4202) to (6.8359, 1.4229) to (6.8357, 1.4245) to (6.8354, 1.4265) to (6.8349, 1.4298) to (6.8345, 1.4330) to (6.8341, 1.4359) to (6.8338, 1.4375) to (6.8335, 1.4397) to (6.8330, 1.4431) to (6.8325, 1.4466) to (6.8321, 1.4489) to (6.8319, 1.4507) to (6.8314, 1.4536) to (6.8309, 1.4572) to (6.8304, 1.4602) to (6.8301, 1.4620) to (6.8298, 1.4645) to (6.8292, 1.4682) to (6.8287, 1.4714) to (6.8284, 1.4734) to (6.8280, 1.4758) to (6.8274, 1.4797) to (6.8269, 1.4827) to (6.8266, 1.4847) to (6.8261, 1.4876) to (6.8254, 1.4916) to (6.8251, 1.4940) to (6.8247, 1.4960) to (6.8241, 1.4999) to (6.8236, 1.5032) to (6.8232, 1.5053) to (6.8227, 1.5084) to (6.8220, 1.5123) to (6.8217, 1.5145) to (6.8212, 1.5171) to (6.8205, 1.5214) to (6.8201, 1.5237) to (6.8197, 1.5261) to (6.8189, 1.5305) to (6.8185, 1.5328) to (6.8181, 1.5353) to (6.8173, 1.5395) to (6.8169, 1.5419) to (6.8164, 1.5449) to (6.8157, 1.5486) to (6.8153, 1.5510) to (6.8146, 1.5547) to (6.8141, 1.5577) to (6.8136, 1.5601) to (6.8129, 1.5642) to (6.8124, 1.5667) to (6.8118, 1.5700) to (6.8112, 1.5732) to (6.8107, 1.5758) to (6.8100, 1.5796) to (6.8095, 1.5823) to (6.8088, 1.5859) to (6.8083, 1.5887) to (6.8078, 1.5916) to (6.8071, 1.5950) to (6.8066, 1.5978) to (6.8059, 1.6013) to (6.8053, 1.6042) to (6.8047, 1.6075) to (6.8041, 1.6104) to (6.8035, 1.6137) to (6.8029, 1.6167) to (6.8022, 1.6199) to (6.8016, 1.6229) to (6.8010, 1.6261) to (6.8004, 1.6291) to (6.7997, 1.6322) to (6.7991, 1.6353) to (6.7985, 1.6383) to (6.7978, 1.6415) to (6.7972, 1.6444) to (6.7966, 1.6476) to (6.7960, 1.6505) to (6.7953, 1.6538) to (6.7947, 1.6566) to (6.7940, 1.6600) to (6.7934, 1.6627) to (6.7927, 1.6661) to (6.7919, 1.6697) to (6.7912, 1.6732) to (6.7900, 1.6785) to (6.7889, 1.6836) to (6.7878, 1.6887) to (6.7867, 1.6937) to (6.7856, 1.6987) to (6.7845, 1.7035) to (6.7834, 1.7083) to (6.7823, 1.7131) to (6.7813, 1.7178) to (6.7802, 1.7224) to (6.7791, 1.7270) to (6.7781, 1.7315) to (6.7770, 1.7360) to (6.7760, 1.7404) to (6.7750, 1.7448) to (6.7739, 1.7492) to (6.7729, 1.7535) to (6.7719, 1.7578) to (6.7708, 1.7621) to (6.7698, 1.7663) to (6.7688, 1.7705) to (6.7678, 1.7747) to (6.7667, 1.7789) to (6.7657, 1.7830) to (6.7647, 1.7872) to (6.7636, 1.7913) to (6.7626, 1.7954) to (6.7616, 1.7995) to (6.7605, 1.8036) to (6.7595, 1.8077) to (6.7584, 1.8118) to (6.7574, 1.8158) to (6.7563, 1.8199) to (6.7553, 1.8240) to (6.7542, 1.8281) to (6.7531, 1.8322) to (6.7520, 1.8363) to (6.7510, 1.8404) to (6.7499, 1.8445) to (6.7487, 1.8487) to (6.7476, 1.8528) to (6.7465, 1.8570) to (6.7454, 1.8612) to (6.7442, 1.8654) to (6.7430, 1.8697) to (6.7414, 1.8756) to (6.6954, 2.0345) to (6.6181, 2.2741) to (6.5391, 2.4923) to (6.4583, 2.6946) to (6.3757, 2.8839) to (6.2911, 3.0628) to (6.2046, 3.2329) to (6.1161, 3.3954) to (6.0255, 3.5514) to (5.9329, 3.7015) to (5.8380, 3.8463) to (5.7410, 3.9863) to (5.6418, 4.1219) to (5.5401, 4.2534) to (5.4363, 4.3810) to (5.3299, 4.5050) to (5.2211, 4.6255) to (5.1099, 4.7425) to (4.9961, 4.8563) to (4.8799, 4.9668) to (4.7609, 5.0742) to (4.6394, 5.1784) to (4.5153, 5.2795) to (4.3885, 5.3774) to (4.2590, 5.4720) to (4.1269, 5.5635) to (3.9921, 5.6516) to (3.8547, 5.7364) to (3.7146, 5.8177) to (3.5720, 5.8955) to (3.4268, 5.9697) to (3.2791, 6.0402) to (3.1290, 6.1069) to (2.9765, 6.1696) to (2.8217, 6.2283) to (2.6648, 6.2829) to (2.5059, 6.3332) to (2.3451, 6.3791) to (2.1824, 6.4206) to (2.0182, 6.4574) to (1.8526, 6.4896) to (1.6857, 6.5170) to (1.5177, 6.5396) to (1.3489, 6.5572) to (1.1795, 6.5699) to (1.0097, 6.5775) to (0.8398, 6.5800) to (0.6699, 6.5775) to (0.5005, 6.5699) to (0.3316, 6.5572) to (0.1636, 6.5394) to (0.0263, 6.5211) to (-0.2031, 6.4827) to (-0.2150, 6.4804) to (-0.2967, 6.4641) to (-0.3842, 6.4453) to (-0.4750, 6.4241) to (-0.5557, 6.4040) to (-0.6472, 6.3795) to (-0.7265, 6.3570) to (-0.8132, 6.3308) to (-0.8912, 6.3060) to (-0.9730, 6.2784) to (-1.0496, 6.2514) to (-1.1269, 6.2227) to (-1.2020, 6.1936) to (-1.2749, 6.1641) to (-1.3485, 6.1331) to (-1.4171, 6.1030) to (-1.4892, 6.0701) to (-1.5537, 6.0395) to (-1.6243, 6.0049) to (-1.6849, 5.9740) to (-1.7540, 5.9378) to (-1.8110, 5.9068) to (-1.8663, 5.8760) to (-1.9320, 5.8381) to (-1.9833, 5.8077) to (-2.0481, 5.7681) to (-2.0962, 5.7379) to (-2.1595, 5.6970) to (-2.2046, 5.6669) to (-2.2527, 5.6343) to (-2.3088, 5.5952) to (-2.3495, 5.5661) to (-2.4089, 5.5226) to (-2.4470, 5.4939) to (-2.4894, 5.4614) to (-2.5406, 5.4212) to (-2.5749, 5.3937) to (-2.6266, 5.3513) to (-2.6628, 5.3209) to (-2.6937, 5.2945) to (-2.7473, 5.2476) to (-2.7763, 5.2217) to (-2.8065, 5.1943) to (-2.8558, 5.1486) to (-2.8819, 5.1239) to (-2.9117, 5.0953) to (-2.9569, 5.0510) to (-2.9805, 5.0273) to (-3.0068, 5.0007) to (-3.0509, 4.9550) to (-3.0726, 4.9321) to (-3.0932, 4.9100) to (-3.1330, 4.8668) to (-3.1588, 4.8381) to (-3.1775, 4.8171) to (-3.2077, 4.7826) to (-3.2396, 4.7454) to (-3.2566, 4.7253) to (-3.2759, 4.7022) to (-3.3078, 4.6635) to (-3.3310, 4.6347) to (-3.3459, 4.6159) to (-3.3675, 4.5885) to (-3.3955, 4.5523) to (-3.4146, 4.5272) to (-3.4278, 4.5097) to (-3.4481, 4.4824) to (-3.4728, 4.4485) to (-3.4914, 4.4226) to (-3.5030, 4.4063) to (-3.5133, 4.3918) to (-3.5248, 4.3753) to (-3.5360, 4.3590) to (-3.5415, 4.3509) to (-3.5469, 4.3429) to (-3.5577, 4.3270) to (-3.5681, 4.3113) to (-3.5771, 4.2977) to (-3.5821, 4.2900) to (-3.5883, 4.2805) to (-3.5980, 4.2654) to (-3.6075, 4.2504) to (-3.6163, 4.2365) to (-3.6208, 4.2292) to (-3.6258, 4.2211) to (-3.6347, 4.2067) to (-3.6434, 4.1925) to (-3.6518, 4.1785) to (-3.6579, 4.1684) to (-3.6620, 4.1615) to (-3.6682, 4.1509) to (-3.6761, 4.1374) to (-3.6838, 4.1241) to (-3.6914, 4.1109) to (-3.6971, 4.1009) to (-3.7007, 4.0944) to (-3.7060, 4.0850) to (-3.7131, 4.0723) to (-3.7200, 4.0597) to (-3.7268, 4.0474) to (-3.7334, 4.0351) to (-3.7374, 4.0278) to (-3.7406, 4.0217) to (-3.7462, 4.0111) to (-3.7524, 3.9993) to (-3.7585, 3.9877) to (-3.7645, 3.9761) to (-3.7693, 3.9668) to (-3.7721, 3.9612) to (-3.7743, 3.9570) to (-3.7760, 3.9535) to (-3.7778, 3.9501) to (-3.7792, 3.9472) to (-3.7817, 3.9423) to (-3.7841, 3.9375) to (-3.7861, 3.9335) to (-3.7888, 3.9280) to (-3.7909, 3.9239) to (-3.7935, 3.9185) to (-3.7955, 3.9145) to (-3.7978, 3.9097) to (-3.8001, 3.9051) to (-3.8020, 3.9012) to (-3.8045, 3.8959) to (-3.8064, 3.8920) to (-3.8089, 3.8868) to (-3.8108, 3.8829) to (-3.8130, 3.8783) to (-3.8149, 3.8744) to (-3.8151, 3.8739) to (-3.8169, 3.8701) to (-3.8193, 3.8650) to (-3.8211, 3.8612) to (-3.8235, 3.8562) to (-3.8252, 3.8524) to (-3.8274, 3.8478) to (-3.8293, 3.8437) to (-3.8310, 3.8400) to (-3.8333, 3.8351) to (-3.8349, 3.8315) to (-3.8371, 3.8266) to (-3.8388, 3.8230) to (-3.8409, 3.8185) to (-3.8426, 3.8146) to (-3.8442, 3.8110) to (-3.8464, 3.8063) to (-3.8480, 3.8028) to (-3.8500, 3.7981) to (-3.8516, 3.7946) to (-3.8521, 3.7934) to (-3.8537, 3.7899) to (-3.8552, 3.7865) to (-3.8567, 3.7830) to (-3.8587, 3.7785) to (-3.8603, 3.7751) to (-3.8622, 3.7706) to (-3.8637, 3.7671) to (-3.8656, 3.7628) to (-3.8671, 3.7593) to (-3.8685, 3.7560) to (-3.8704, 3.7516) to (-3.8719, 3.7483) to (-3.8737, 3.7439) to (-3.8751, 3.7407) to (-3.8769, 3.7364) to (-3.8784, 3.7330) to (-3.8797, 3.7299) to (-3.8815, 3.7256) to (-3.8828, 3.7224) to (-3.8846, 3.7182) to (-3.8859, 3.7150) to (-3.8875, 3.7111) to (-3.8888, 3.7080) to (-3.8890, 3.7077) to (-3.8903, 3.7046) to (-3.8920, 3.7005) to (-3.8932, 3.6974) to (-3.8949, 3.6933) to (-3.8961, 3.6903) to (-3.8978, 3.6862) to (-3.8990, 3.6832) to (-3.9003, 3.6801) to (-3.9018, 3.6762) to (-3.9030, 3.6732) to (-3.9046, 3.6693) to (-3.9058, 3.6663) to (-3.9074, 3.6624) to (-3.9085, 3.6595) to (-3.9098, 3.6564) to (-3.9112, 3.6527) to (-3.9124, 3.6498) to (-3.9139, 3.6460) to (-3.9150, 3.6431) to (-3.9165, 3.6393) to (-3.9176, 3.6365) to (-3.9188, 3.6335) to (-3.9201, 3.6299) to (-3.9212, 3.6271) to (-3.9226, 3.6234) to (-3.9237, 3.6207) to (-3.9242, 3.6194) to (-3.9251, 3.6170) to (-3.9261, 3.6142) to (-3.9273, 3.6113) to (-3.9286, 3.6079) to (-3.9296, 3.6052) to (-3.9310, 3.6016) to (-3.9320, 3.5989) to (-3.9333, 3.5954) to (-3.9343, 3.5927) to (-3.9354, 3.5898) to (-3.9366, 3.5866) to (-3.9376, 3.5839) to (-3.9388, 3.5805) to (-3.9398, 3.5778) to (-3.9411, 3.5744) to (-3.9420, 3.5718) to (-3.9431, 3.5689) to (-3.9442, 3.5659) to (-3.9451, 3.5633) to (-3.9463, 3.5600) to (-3.9473, 3.5574) to (-3.9485, 3.5541) to (-3.9494, 3.5516) to (-3.9504, 3.5488) to (-3.9515, 3.5458) to (-3.9523, 3.5434) to (-3.9535, 3.5401) to (-3.9544, 3.5377) to (-3.9555, 3.5344) to (-3.9564, 3.5320) to (-3.9573, 3.5293) to (-3.9582, 3.5269) to (-3.9584, 3.5264) to (-3.9592, 3.5240) to (-3.9603, 3.5208) to (-3.9611, 3.5185) to (-3.9622, 3.5153) to (-3.9630, 3.5130) to (-3.9640, 3.5102) to (-3.9649, 3.5076) to (-3.9657, 3.5053) to (-3.9668, 3.5021) to (-3.9676, 3.4999) to (-3.9686, 3.4968) to (-3.9694, 3.4945) to (-3.9703, 3.4918) to (-3.9712, 3.4893) to (-3.9720, 3.4870) to (-3.9730, 3.4840) to (-3.9737, 3.4818) to (-3.9747, 3.4788) to (-3.9755, 3.4766) to (-3.9764, 3.4739) to (-3.9772, 3.4715) to (-3.9779, 3.4693) to (-3.9789, 3.4664) to (-3.9796, 3.4642) to (-3.9805, 3.4614) to (-3.9813, 3.4592) to (-3.9821, 3.4565) to (-3.9829, 3.4543) to (-3.9836, 3.4521) to (-3.9845, 3.4493) to (-3.9852, 3.4472) to (-3.9861, 3.4444) to (-3.9868, 3.4423) to (-3.9876, 3.4397) to (-3.9883, 3.4375) to (-3.9890, 3.4354) to (-3.9899, 3.4327) to (-3.9904, 3.4312) to (-3.9908, 3.4300) to (-3.9914, 3.4280) to (-3.9921, 3.4259) to (-3.9929, 3.4233) to (-3.9935, 3.4212) to (-3.9942, 3.4192) to (-3.9950, 3.4166) to (-3.9956, 3.4146) to (-3.9965, 3.4119) to (-3.9971, 3.4100) to (-3.9979, 3.4074) to (-3.9985, 3.4054) to (-3.9991, 3.4034) to (-3.9999, 3.4009) to (-4.0005, 3.3989) to (-4.0013, 3.3964) to (-4.0019, 3.3945) to (-4.0027, 3.3919) to (-4.0041, 3.3875) to (-4.0056, 3.3825) to (-4.0071, 3.3776) to (-4.0086, 3.3726) to (-4.0100, 3.3678) to (-4.0115, 3.3630) to (-4.0129, 3.3582) to (-4.0143, 3.3534) to (-4.0157, 3.3487) to (-4.0171, 3.3441) to (-4.0184, 3.3395) to (-4.0197, 3.3349) to (-4.0208, 3.3313) to (-4.0214, 3.3291) to (-4.0223, 3.3259) to (-4.0236, 3.3214) to (-4.0249, 3.3170) to (-4.0261, 3.3126) to (-4.0273, 3.3083) to (-4.0285, 3.3040) to (-4.0297, 3.2997) to (-4.0309, 3.2955) to (-4.0321, 3.2913) to (-4.0331, 3.2874) to (-4.0343, 3.2831) to (-4.0354, 3.2790) to (-4.0365, 3.2749) to (-4.0376, 3.2709) to (-4.0387, 3.2669) to (-4.0398, 3.2630) to (-4.0408, 3.2591) to (-4.0418, 3.2552) to (-4.0429, 3.2513) to (-4.0439, 3.2475) to (-4.0448, 3.2437) to (-4.0458, 3.2399) to (-4.0468, 3.2362) to (-4.0478, 3.2325) to (-4.0487, 3.2288) to (-4.0493, 3.2263) to (-4.0498, 3.2245) to (-4.0506, 3.2216) to (-4.0515, 3.2180) to (-4.0524, 3.2144) to (-4.0532, 3.2109) to (-4.0541, 3.2074) to (-4.0550, 3.2039) to (-4.0558, 3.2005) to (-4.0567, 3.1971) to (-4.0575, 3.1937) to (-4.0584, 3.1903) to (-4.0675, 3.1528) to (-4.0879, 3.0607) to (-4.1095, 2.9464) to (-4.1277, 2.8283) to (-4.1424, 2.7066) to (-4.1530, 2.5815) to (-4.1593, 2.4529) to (-4.1609, 2.3228) to (-4.1577, 2.1891) to (-4.1492, 2.0538) to (-4.1354, 1.9169) to (-4.1160, 1.7791) to (-4.0910, 1.6409) to (-4.0603, 1.5029) to (-4.0239, 1.3656) to (-3.9820, 1.2296) to (-3.9348, 1.0955) to (-3.8824, 0.9638) to (-3.8251, 0.8351) to (-3.7688, 0.7218) to (-3.7386, 0.6677) to (-3.7328, 0.6569) to (-3.7295, 0.6508) to (-3.7253, 0.6433) to (-3.7185, 0.6309) to (-3.7115, 0.6183) to (-3.7044, 0.6056) to (-3.6971, 0.5927) to (-3.6896, 0.5796) to (-3.6819, 0.5664) to (-3.6741, 0.5530) to (-3.6663, 0.5397) to (-3.6622, 0.5330) to (-3.6580, 0.5257) to (-3.6496, 0.5118) to (-3.6410, 0.4978) to (-3.6323, 0.4835) to (-3.6233, 0.4691) to (-3.6141, 0.4545) to (-3.6047, 0.4397) to (-3.5955, 0.4254) to (-3.5906, 0.4180) to (-3.5852, 0.4096) to (-3.5752, 0.3942) to (-3.5648, 0.3787) to (-3.5542, 0.3629) to (-3.5434, 0.3470) to (-3.5323, 0.3308) to (-3.5217, 0.3157) to (-3.5159, 0.3076) to (-3.5092, 0.2979) to (-3.4973, 0.2812) to (-3.4850, 0.2642) to (-3.4725, 0.2471) to (-3.4596, 0.2297) to (-3.4465, 0.2121) to (-3.4397, 0.2036) to (-3.4329, 0.1943) to (-3.4190, 0.1762) to (-3.4048, 0.1580) to (-3.3902, 0.1395) to (-3.3752, 0.1208) to (-3.3642, 0.1077) to (-3.3564, 0.0981) to (-3.3441, 0.0826) to (-3.3279, 0.0630) to (-3.3114, 0.0429) to (-3.2943, 0.0214) to (-3.2828, 0.0111) to (-3.2767,0.0000) to (-3.2667,0.0000) to (-3.2626,0.0000) to (-3.2526,0.0000) to (-3.2444,0.0000) to (-3.2344,0.0000) to (-3.2264,0.0000) to (-3.2222,0.0000) to (-3.2122,0.0000) to (-3.2044,0.0000) to (-3.1944,0.0000) to (-3.1868,0.0000) to (-3.1818,0.0000) to (-3.1718,0.0000) to (-3.1644,0.0000) to (-3.1544,0.0000) to (-3.1472,0.0000) to (-3.1414,0.0000) to (-3.1314,0.0000) to (-3.1244,0.0000) to (-3.1144,0.0000) to (-3.1120,0.0000) to (-3.1020,0.0000) to (-3.1010,0.0000) to (-3.0910,0.0000) to (-3.0844,0.0000) to (-3.0744,0.0000) to (-3.0680,0.0000) to (-3.0606,0.0000) to (-3.0444, 0.0000) to (-3.0283, 0.0000) to (-3.0202, 0.0000) to (-3.0044, 0.0000) to (-2.9887, 0.0000) to (-2.9798, 0.0000) to (-2.9644, 0.0000) to (-2.9509, 0.0000) to (-2.9394, 0.0000) to (-2.9243, 0.0000) to (-2.9094, 0.0000) to (-2.8990, 0.0000) to (-2.8843, 0.0000) to (-2.8697, 0.0000) to (-2.8586, 0.0000) to (-2.8442, 0.0000) to (-2.8300, 0.0000) to (-2.8182, 0.0000) to (-2.8071, 0.0101) to (-2.7936, 0.0267) to (-2.7767, 0.0482) to (-2.7623, 0.0665) to (-2.7534, 0.0773) to (-2.7414, 0.0903) to (-2.7229, 0.1116) to (-2.7065, 0.1304) to (-2.6968, 0.1414) to (-2.6841, 0.1547) to (-2.6638, 0.1767) to (-2.6478, 0.1941) to (-2.6371, 0.2053) to (-2.6212, 0.2213) to (-2.5989, 0.2439) to (-2.5859, 0.2575) to (-2.5742, 0.2686) to (-2.5522, 0.2900) to (-2.5330, 0.3085) to (-2.5206, 0.3203) to (-2.5024, 0.3369) to (-2.4786, 0.3586) to (-2.4654, 0.3708) to (-2.4495, 0.3845) to (-2.4226, 0.4079) to (-2.4085, 0.4203) to (-2.3931, 0.4329) to (-2.3649, 0.4563) to (-2.3499, 0.4688) to (-2.3332, 0.4818) to (-2.3055, 0.5038) to (-2.2895, 0.5163) to (-2.2696, 0.5312) to (-2.2443, 0.5502) to (-2.2275, 0.5626) to (-2.2020, 0.5807) to (-2.1814, 0.5955) to (-2.1636, 0.6078) to (-2.1352, 0.6272) to (-2.1167, 0.6397) to (-2.0929, 0.6551) to (-2.0697, 0.6703) to (-2.0502, 0.6824) to (-2.0224, 0.6997) to (-2.0024, 0.7120) to (-1.9750, 0.7281) to (-1.9543, 0.7404) to (-1.9323, 0.7527) to (-1.9060, 0.7677) to (-1.8843, 0.7795) to (-1.8576, 0.7940) to (-1.8352, 0.8057) to (-1.8089, 0.8193) to (-1.7860, 0.8309) to (-1.7601, 0.8436) to (-1.7365, 0.8550) to (-1.7110, 0.8669) to (-1.6869, 0.8782) to (-1.6618, 0.8893) to (-1.6370, 0.9003) to (-1.6123, 0.9108) to (-1.5870, 0.9215) to (-1.4274, 0.9729) to (-1.0454, 0.9979) to (-0.5404, 0.7895) to (-0.3900, 0.6494) to (-0.3867, 0.6456) to (-0.3828, 0.6414) to (-0.3795, 0.6377) to (-0.3754, 0.6333) to (-0.3720, 0.6297) to (-0.3677, 0.6251) to (-0.3631, 0.6204) to (-0.3584, 0.6157) to (-0.3512, 0.6086) to (-0.3439, 0.6016) to (-0.3365, 0.5946) to (-0.3289, 0.5877) to (-0.3211, 0.5807) to (-0.3130, 0.5738) to (-0.3048, 0.5668) to (-0.2962, 0.5597) to (-0.2873, 0.5525) to (-0.2777, 0.5449) to (-0.2674, 0.5368) to (-0.2556, 0.5278) to (-0.2413, 0.5169) to (-0.2218, 0.5018) to (-0.1894, 0.4754) to (-0.1152, 0.4027) to (0.0088, 0.1901) to (0.0338, 0.0897) to (0.0353, 0.0802) to (0.0356, 0.0778) to (0.0360, 0.0754) to (0.0363, 0.0730) to (0.0367, 0.0706) to (0.0371, 0.0682) to (0.0374, 0.0658) to (0.0378, 0.0634) to (0.0381, 0.0610) to (0.0385, 0.0586) to (0.0389, 0.0563) to (0.0392, 0.0539) to (0.0396, 0.0515) to (0.0400, 0.0492) to (0.0404, 0.0468) to (0.0407, 0.0444) to (0.0411, 0.0420) to (0.0415, 0.0396) to (0.0419, 0.0372) to (0.0423, 0.0348) to (0.0427, 0.0324) to (0.0431, 0.0299) to (0.0435, 0.0275) to (0.0439, 0.0250) to (0.0443, 0.0225) to (0.0447, 0.0200) to (0.0451, 0.0174) to (0.0455, 0.0148) to (0.0460, 0.0122) to (0.0464, 0.0094) to (0.0468, 0.0065) to cycle; \begin{scope}[yscale=-1] \draw[fill=DutchBlue!80](0.0473, 0.0031) to (0.0475, 0.0000) to (0.0468, 0.0000) to (0.0484, 0.0000) to (0.0500, 0.0000) to (0.0515, 0.0000) to (0.0531, 0.0000) to (0.0547, 0.0000) to (0.0563, 0.0000) to (0.0583, 0.0000) to (0.0598, 0.0000) to (0.0614, 0.0000) to (0.0630, 0.0000) to (0.0646, 0.0000) to (0.0662, 0.0000) to (0.0677, 0.0000) to (0.0693, 0.0000) to (0.0709, 0.0000) to (0.0725, 0.0000) to (0.0741, 0.0000) to (0.0757, 0.0000) to (0.0773, 0.0000) to (0.0788, 0.0000) to (0.0804, 0.0000) to (0.0820, 0.0000) to (0.0836, 0.0000) to (0.0852, 0.0000) to (0.0867, 0.0000) to (0.0883, 0.0000) to (0.0899, 0.0000) to (0.0915, 0.0000) to (0.0931, 0.0000) to (0.0947, 0.0000) to (0.0962, 0.0000) to (0.0978, 0.0000) to (0.0994, 0.0000) to (0.1010, 0.0000) to (0.1026, 0.0000) to (0.1042, 0.0000) to (0.1058, 0.0000) to (0.1074, 0.0000) to (0.1089, 0.0000) to (0.1105, 0.0000) to (0.1121, 0.0000) to (0.1137, 0.0000) to (0.1153, 0.0000) to (0.1169, 0.0000) to (0.1185, 0.0000) to (0.1201, 0.0000) to (0.1218, 0.0000) to (0.1234, 0.0000) to (0.1250, 0.0000) to (0.1266, 0.0000) to (0.1282, 0.0000) to (0.1298, 0.0000) to (0.1314, 0.0000) to (0.1330, 0.0000) to (0.1346, 0.0000) to (0.1362, 0.0000) to (0.1378, 0.0000) to (0.1394, 0.0000) to (0.1410, 0.0000) to (0.1426, 0.0000) to (0.1442, 0.0000) to (0.1458, 0.0000) to (0.1474, 0.0000) to (0.1490, 0.0000) to (0.1506, 0.0000) to (0.1522, 0.0000) to (0.1544, 0.0000) to (0.1561, 0.0000) to (0.1577, 0.0000) to (0.1593, 0.0000) to (0.1609, 0.0000) to (0.1625, 0.0000) to (0.1641, 0.0000) to (0.1657, 0.0000) to (0.1673, 0.0000) to (0.1689, 0.0000) to (0.1706, 0.0000) to (0.1722, 0.0000) to (0.1738, 0.0000) to (0.1754, 0.0000) to (0.1770, 0.0000) to (0.1787, 0.0000) to (0.1803, 0.0000) to (0.1819, 0.0000) to (0.1835, 0.0000) to (0.1852, 0.0000) to (0.1868, 0.0000) to (0.1884, 0.0000) to (0.1900, 0.0000) to (0.1917, 0.0000) to (0.1933, 0.0000) to (0.1949, 0.0000) to (0.1965, 0.0000) to (0.1982, 0.0000) to (0.1998, 0.0000) to (0.2014, 0.0000) to (0.2031, 0.0000) to (0.2047, 0.0000) to (0.2064, 0.0000) to (0.2080, 0.0000) to (0.2096, 0.0000) to (0.2113, 0.0000) to (0.2129, 0.0000) to (0.2146, 0.0000) to (0.2162, 0.0000) to (0.2178, 0.0000) to (0.2195, 0.0000) to (0.2211, 0.0000) to (0.2228, 0.0000) to (0.2244, 0.0000) to (0.2261, 0.0000) to (0.2277, 0.0000) to (0.2294, 0.0000) to (0.2310, 0.0000) to (0.2327, 0.0000) to (0.2344, 0.0000) to (0.2360, 0.0000) to (0.2377, 0.0000) to (0.2393, 0.0000) to (0.2410, 0.0000) to (0.2427, 0.0000) to (0.2443, 0.0000) to (0.2460, 0.0000) to (0.2477, 0.0000) to (0.2493, 0.0000) to (0.2510, 0.0000) to (0.2527, 0.0000) to (0.2543, 0.0000) to (0.2560, 0.0000) to (0.2577, 0.0000) to (0.2594, 0.0000) to (0.2610, 0.0000) to (0.2627, 0.0000) to (0.2644, 0.0000) to (0.2661, 0.0000) to (0.2678, 0.0000) to (0.2705, 0.0000) to (0.2722, 0.0000) to (0.2738, 0.0000) to (0.2755, 0.0000) to (0.2772, 0.0000) to (0.2789, 0.0000) to (0.2806, 0.0000) to (0.2823, 0.0000) to (0.2840, 0.0000) to (0.2857, 0.0000) to (0.2874, 0.0000) to (0.2891, 0.0000) to (0.2908, 0.0000) to (0.2925, 0.0000) to (0.2942, 0.0000) to (0.2959, 0.0000) to (0.2976, 0.0000) to (0.2993, 0.0000) to (0.3011, 0.0000) to (0.3028, 0.0000) to (0.3045, 0.0000) to (0.3062, 0.0000) to (0.3080, 0.0000) to (0.3097, 0.0000) to (0.3114, 0.0000) to (0.3131, 0.0000) to (0.3149, 0.0000) to (0.3166, 0.0000) to (0.3183, 0.0000) to (0.3200, 0.0000) to (0.3256, 0.0112) to (0.3299, 0.0194) to (0.3343, 0.0273) to (0.3536, 0.0513) to (0.4149, 0.0769) to (0.4541, 0.0744) to (0.4818, 0.0668) to (0.5041, 0.0577) to (0.5232, 0.0482) to (0.5405, 0.0381) to (0.5562, 0.0279) to (0.5711, 0.0170) to (0.5852, 0.0015) to (0.5932, 0.0000) to (0.5954, 0.0000) to (0.5975, 0.0000) to (0.5996, 0.0000) to (0.6018, 0.0000) to (0.6039, 0.0000) to (0.6060, 0.0000) to (0.6082, 0.0000) to (0.6116, 0.0000) to (0.6138, 0.0000) to (0.6159, 0.0000) to (0.6181, 0.0000) to (0.6203, 0.0000) to (0.6224, 0.0000) to (0.6246, 0.0000) to (0.6268, 0.0000) to (0.6290, 0.0000) to (0.6312, 0.0000) to (0.6334, 0.0000) to (0.6356, 0.0000) to (0.6378, 0.0000) to (0.6400, 0.0000) to (0.6422, 0.0000) to (0.6444, 0.0000) to (0.6467, 0.0000) to (0.6489, 0.0000) to (0.6511, 0.0000) to (0.6534, 0.0000) to (0.6560, 0.0000) to (0.6582, 0.0000) to (0.6605, 0.0000) to (0.6627, 0.0000) to (0.6650, 0.0000) to (0.6673, 0.0000) to (0.6695, 0.0000) to (0.6718, 0.0000) to (0.6741, 0.0000) to (0.6764, 0.0000) to (0.6781, 0.0000) to (0.6804, 0.0000) to (0.6827, 0.0000) to (0.6850, 0.0000) to (0.6873, 0.0000) to (0.6896, 0.0000) to (0.6919, 0.0000) to (0.6943, 0.0000) to (0.6966, 0.0000) to (0.6989, 0.0000) to (0.7013, 0.0000) to (0.7036, 0.0000) to (0.7060, 0.0000) to (0.7083, 0.0000) to (0.7107, 0.0000) to (0.7130, 0.0000) to (0.7154, 0.0000) to (0.7178, 0.0000) to (0.7202, 0.0000) to (0.7226, 0.0000) to (0.7250, 0.0000) to (0.7274, 0.0000) to (0.7298, 0.0000) to (0.7322, 0.0000) to (0.7346, 0.0000) to (0.7370, 0.0000) to (0.7394, 0.0000) to (0.7419, 0.0000) to (0.7443, 0.0000) to (0.7468, 0.0000) to (0.7492, 0.0000) to (0.7517, 0.0000) to (0.7541, 0.0000) to (0.7566, 0.0000) to (0.7658, 0.0137) to (0.7742, 0.0264) to (0.7825, 0.0385) to (0.7903, 0.0503) to (0.7978, 0.0619) to (0.8051, 0.0734) to (0.8119, 0.0846) to (0.8185, 0.0958) to (0.8226, 0.1032) to (0.8263, 0.1098) to (0.8293, 0.1154) to (0.8324, 0.1209) to (0.8355, 0.1270) to (0.8382, 0.1321) to (0.8413, 0.1382) to (0.8438, 0.1433) to (0.8466, 0.1490) to (0.8490, 0.1540) to (0.8515, 0.1593) to (0.8686, 0.1925) to (1.3106, 0.3934) to (1.5205, 0.2856) to (1.5326, 0.2742) to (1.5451, 0.2623) to (1.5568, 0.2510) to (1.5694, 0.2387) to (1.5808, 0.2276) to (1.5934, 0.2147) to (1.6045, 0.2039) to (1.6173, 0.1903) to (1.6280, 0.1798) to (1.6386, 0.1682) to (1.6513, 0.1554) to (1.6614, 0.1442) to (1.6744, 0.1305) to (1.6842, 0.1199) to (1.6974, 0.1049) to (1.7069, 0.0951) to (1.7172, 0.0825) to (1.7293, 0.0697) to (1.7383, 0.0589) to (1.7517, 0.0427) to (1.7603, 0.0339) to (1.7702, 0.0181) to (1.7822, 0.0055) to (1.7870, 0.0000) to (1.7936, 0.0000) to (1.8002, 0.0000) to (1.8040, 0.0000) to (1.8107, 0.0000) to (1.8175, 0.0000) to (1.8242, 0.0000) to (1.8311, 0.0000) to (1.8379, 0.0000) to (1.8442, 0.0000) to (1.8493, 0.0000) to (1.8563, 0.0000) to (1.8633, 0.0000) to (1.8703, 0.0000) to (1.8774, 0.0000) to (1.8844, 0.0000) to (1.8916, 0.0000) to (1.8988, 0.0000) to (1.9061, 0.0000) to (1.9134, 0.0000) to (1.9207, 0.0000) to (1.9213, 0.0000) to (1.9246, 0.0000) to (1.9320, 0.0000) to (1.9395, 0.0000) to (1.9470, 0.0000) to (1.9545, 0.0000) to (1.9621, 0.0000) to (1.9648, 0.0000) to (1.9725, 0.0000) to (1.9802, 0.0000) to (1.9879, 0.0000) to (1.9957, 0.0000) to (1.9979, 0.0000) to (2.0050, 0.0000) to (2.0129, 0.0000) to (2.0209, 0.0000) to (2.0289, 0.0000) to (2.0370, 0.0000) to (2.0451, 0.0000) to (2.0452, 0.0000) to (2.0534, 0.0000) to (2.0616, 0.0000) to (2.0699, 0.0000) to (2.0782, 0.0000) to (2.0794, 0.0000) to (2.0854, 0.0000) to (2.0939, 0.0000) to (2.1023, 0.0000) to (2.1109, 0.0000) to (2.1195, 0.0000) to (2.1256, 0.0000) to (2.1343, 0.0000) to (2.1431, 0.0000) to (2.1519, 0.0000) to (2.1608, 0.0000) to (2.1658, 0.0000) to (2.1665, 0.0000) to (2.1754, 0.0000) to (2.1951, 0.0228) to (2.2061, 0.0391) to (2.2142, 0.0483) to (2.2274, 0.0638) to (2.2416, 0.0818) to (2.2493, 0.0919) to (2.2581, 0.1022) to (2.2729, 0.1209) to (2.2838, 0.1353) to (2.2909, 0.1445) to (2.3013, 0.1576) to (2.3150, 0.1756) to (2.3245, 0.1886) to (2.3310, 0.1973) to (2.3413, 0.2110) to (2.3540, 0.2283) to (2.3637, 0.2419) to (2.3698, 0.2505) to (2.3784, 0.2624) to (2.3902, 0.2791) to (2.4016, 0.2956) to (2.4073, 0.3039) to (2.4128, 0.3119) to (2.4238, 0.3280) to (2.4344, 0.3438) to (2.4495, 0.3663) to (2.4661, 0.3901) to (2.4884, 0.4194) to (2.5271, 0.4669) to (2.5705, 0.5147) to (2.6163, 0.5605) to (2.6427, 0.5852) to (2.6748, 0.6126) to (2.7383, 0.6629) to (2.8118, 0.7138) to (2.8975, 0.7644) to (2.9685, 0.8006) to (3.0232, 0.8244) to (3.1183, 0.8584) to (3.2621, 0.8948) to (3.4362, 0.9147) to (3.6487, 0.9030) to (3.8420, 0.8562) to (3.9872, 0.7927) to (4.1934, 0.6442) to (4.2652, 0.5714) to (4.2932, 0.5399) to (4.3194, 0.5092) to (4.3441, 0.4794) to (4.3584, 0.4618) to (4.3698, 0.4473) to (4.3892, 0.4220) to (4.4098, 0.3945) to (4.4292, 0.3678) to (4.4475, 0.3418) to (4.4616, 0.3214) to (4.4699, 0.3091) to (4.4761, 0.2999) to (4.4810, 0.2924) to (4.4859, 0.2850) to (4.4898, 0.2789) to (4.4965, 0.2683) to (4.5029, 0.2584) to (4.5083, 0.2497) to (4.5153, 0.2384) to (4.5205, 0.2300) to (4.5271, 0.2190) to (4.5321, 0.2109) to (4.5378, 0.2010) to (4.5431, 0.1922) to (4.5477, 0.1842) to (4.5536, 0.1739) to (4.5580, 0.1662) to (4.5636, 0.1561) to (4.5678, 0.1488) to (4.5727, 0.1398) to (4.5767, 0.1327) to (4.5772, 0.1317) to (4.5811, 0.1243) to (4.5861, 0.1150) to (4.5899, 0.1080) to (4.5947, 0.0988) to (4.5982, 0.0921) to (4.6025, 0.0834) to (4.6063, 0.0765) to (4.6096, 0.0696) to (4.6139, 0.0612) to (4.6171, 0.0547) to (4.6212, 0.0462) to (4.6243, 0.0402) to (4.6280, 0.0318) to (4.6312, 0.0259) to (4.6340, 0.0190) to (4.6378, 0.0117) to (4.6405, 0.0047) to (4.6426, 0.0000) to (4.6583, 0.0000) to (4.6667, 0.0000) to (4.6684, 0.0000) to (4.6750, 0.0) to (4.685, 0.0) to (4.6970, 0.0000) to (4.6985, 0.0000) to (4.7050, 0.0) to (4.7150, 0.0) to (4.7273, 0.0000) to (4.7300, 0.0) to (4.7387, 0.0000) to (4.74, 0.0) to (4.75, 0.0) to (4.7576, 0.0000) to (4.76, 0.0) to (4.77, 0.0) to (4.7789, 0.0000) to (4.7879, 0.0000) to (4.795, 0.0) to (4.805, 0.0) to (4.81,0.0) to (4.8182, 0.0000) to (4.8191,0.0000)
to (4.8291,0.0000)
to (4.8391,0.0000)
to (4.8485,0.0000)
to (4.8585,0.0000)
to (4.8593,0.0000)
to (4.8693,0.0000)
to (4.8788,0.0000)
to (4.8888,0.0000)
to (4.8988,0.0000)
to (4.8995,0.0000)
to (4.9091,0.0000)
to (4.9191,0.0000)
to (4.9291,0.0000)
to (4.9391,0.0000)
to (4.9394,0.0000)
to (4.9397,0.0000)
to (4.9497,0.0000)
to (4.9597,0.0000)
to (4.9697,0.0000)
to (4.9797,0.0000)
to (4.9799,0.0000)
to (4.9899,0.0000)
to (4.9999,0.0000)
to (5.0000,0.0000)
to (5.0100,0.0000)
to (5.0200,0.0000)
to (5.0201,0.0000)
to (5.0301,0.0000)
to (5.0303,0.0000)
to (5.0403,0.0000)
to (5.0503,0.0000)
to (5.0577,0.0000)
to (5.0603,0.0000)
to (5.0606,0.0000)
to (5.0706,0.0000)
to (5.0806,0.0000)
to (5.0906,0.0000)
to (5.0909,0.0000)
to (5.1005,0.0000)
to (5.1105,0.0000)
to (5.1205,0.0000)
to (5.1212,0.0000)
to (5.1312,0.0000)
to (5.1407,0.0000)
to (5.1507,0.0000)
to (5.1515,0.0000)
to (5.1615,0.0000)
to (5.1715,0.0000)
to (5.1809,0.0000)
to (5.1818,0.0000)
to (5.1918,0.0000)
to (5.2018,0.0000)
to (5.2118,0.0000)
to (5.2121,0.0000)
to (5.2211,0.0000)
to (5.2311,0.0000)
to (5.2411,0.0000)
to (5.2424,0.0000)
to (5.2524,0.0000)
to (5.2613,0.0000)
to (5.2713,0.0000)
to (5.2727,0.0000)
to (5.2827,0.0000)
to (5.2927,0.0000)
to (5.3015,0.0000)
to (5.3030,0.0000)
to (5.3130,0.0000)
to (5.3230,0.0000)
to (5.3330,0.0000)
to (5.3333,0.0000)
to (5.3417,0.0000)
to (5.3517,0.0000)
to (5.3617,0.0000)
to (5.3636,0.0000)
to (5.3736,0.0000)
to (5.3819,0.0000)
to (5.3919,0.0000)
to (5.3939,0.0000)
to (5.4039,0.0000)
to (5.4139,0.0000)
to (5.4221,0.0000)
to (5.4242,0.0000)
to (5.4342,0.0000)
to (5.4442,0.0000)
to (5.4542,0.0000)
to (5.4545,0.0000)
to (5.4623,0.0000)
to (5.4723,0.0000)
to (5.4823,0.0000)
to (5.4848,0.0000)
to (5.4948,0.0000)
to (5.5025,0.0000)
to (5.5125,0.0000)
to (5.5147,0.0000)
to (5.5152,0.0000)
to (5.5252,0.0000)
to (5.5352,0.0000)
to (5.5427,0.0000)
to (5.5455,0.0000)
to (5.5555,0.0000)
to (5.5655,0.0000)
to (5.5755,0.0000)
to (5.5758,0.0000)
to (5.5829,0.0000)
to (5.5929,0.0000)
to (5.6029,0.0000)
to (5.6061,0.0000)
to (5.6161,0.0000)
to (5.6231,0.0000)
to (5.6331,0.0000)
to (5.6364,0.0000)
to (5.6464,0.0000)
to (5.6564,0.0000)
to (5.6633,0.0000)
to (5.6667,0.0000)
to (5.6767,0.0000)
to (5.6867,0.0000)
to (5.6967,0.0000)
to (5.6970,0.0000)
to (5.7035,0.0000)
to (5.7135,0.0000)
to (5.7235,0.0000)
to (5.7273,0.0000)
to (5.7373,0.0000)
to (5.7437,0.0000)
to (5.7537,0.0000)
to (5.7576,0.0000)
to (5.7676,0.0000)
to (5.7776,0.0000)
to (5.7839,0.0000)
to (5.7879,0.0000)
to (5.7979,0.0000)
to (5.8079,0.0000)
to (5.8179,0.0000)
to (5.8182,0.0000)
to (5.8241,0.0000)
to (5.8341,0.0000)
to (5.8441,0.0000)
to (5.8485,0.0000)
to (5.8585,0.0000)
to (5.8643,0.0000)
to (5.8743,0.0000)
to (5.8788,0.0000)
to (5.8888,0.0000)
to (5.8988,0.0000)
to (5.9045,0.0000)
to (5.9091,0.0000)
to (5.9191,0.0000)
to (5.9291,0.0000)
to (5.9391,0.0000)
to (5.9394,0.0000)
to (5.9447,0.0000)
to (5.9547,0.0000)
to (5.9647,0.0000)
to (5.9697,0.0000)
to (5.9797,0.0000)
to (5.9849,0.0000)
to (5.9949,0.0000)
to (6.0000,0.0000)
to (6.0100,0.0000)
to (6.0200,0.0000)
to (6.0251,0.0000)
to (6.0303,0.0000)
to (6.0403,0.0000)
to (6.0503,0.0000)
to (6.0590,0.0000)
to (6.0606,0.0000)
to (6.0653,0.0000)
to (6.0753,0.0000)
to (6.0853,0.0000)
to (6.0909,0.0000)
to (6.1009,0.0000)
to (6.1055,0.0000)
to (6.1155,0.0000)
to (6.1212,0.0000)
to (6.1312,0.0000)
to (6.1412,0.0000)
to (6.1457,0.0000)
to (6.1515,0.0000)
to (6.1615,0.0000)
to (6.1715,0.0000)
to (6.1815,0.0000)
to (6.1818,0.0000)
to (6.1859,0.0000)
to (6.1959,0.0000)
to (6.2059,0.0000)
to (6.2121,0.0000)
to (6.2221,0.0000)
to (6.2261,0.0000)
to (6.2361,0.0000)
to (6.2424,0.0000)
to (6.2524,0.0000)
to (6.2624,0.0000)
to (6.2663,0.0000)
to (6.2727,0.0000)
to (6.2827,0.0000)
to (6.2927,0.0000)
to (6.3027,0.0000)
to (6.3030,0.0000)
to (6.3065,0.0000)
to (6.3165,0.0000)
to (6.3265,0.0000)
to (6.3333,0.0000)
to (6.3433,0.0000)
to (6.3467,0.0000)
to (6.3567,0.0000)
to (6.3636,0.0000)
to (6.3736,0.0000)
to (6.3836,0.0000)
to (6.3869,0.0000)
to (6.3939,0.0000)
to (6.4039,0.0000)
to (6.4139,0.0000)
to (6.4239,0.0000)
to (6.4242,0.0000)
to (6.4271,0.0000)
to (6.4371,0.0000)
to (6.4471,0.0000)
to (6.4545,0.0000)
to (6.4645,0.0000)
to (6.4673,0.0000)
to (6.4773,0.0000)
to (6.4848,0.0000)
to (6.4948,0.0000)
to (6.5048,0.0000)
to (6.5075,0.0000)
to (6.5152,0.0000)
to (6.5252,0.0000)
to (6.5352,0.0000)
to (6.5452,0.0000)
to (6.5455,0.0000)
to (6.5477,0.0000)
to (6.5577,0.0000)
to (6.5677,0.0000)
to (6.5758,0.0000)
to (6.5858,0.0000)
to (6.5879,0.0000)
to (6.5979,0.0000)
to (6.6061,0.0000)
to (6.6161,0.0000)
to (6.6261,0.0000)
to (6.6281,0.0000)
to (6.6364,0.0000)
to (6.6464,0.0000)
to (6.6564,0.0000)
to (6.6664,0.0000)
to (6.6667,0.0000)
to (6.6683,0.0000)
to (6.6783,0.0000)
to (6.6883,0.0000)
to (6.6970,0.0000)
to (6.7070,0.0000)
to (6.7085,0.0000)
to (6.7185,0.0000)
to (6.7187,0.0000)
to (6.7273,0.0000)
to (6.7373,0.0000)
to (6.7473,0.0000)
to (6.7487,0.0000) to (6.7563, 0.0012) to (6.7573, 0.0082) to (6.7582, 0.0110) to (6.7594, 0.0163) to (6.7603, 0.0198) to (6.7615, 0.0245) to (6.7624, 0.0281) to (6.7636, 0.0325) to (6.7644, 0.0362) to (6.7653, 0.0395) to (6.7664, 0.0441) to (6.7672, 0.0474) to (6.7683, 0.0518) to (6.7691, 0.0552) to (6.7702, 0.0594) to (6.7720, 0.0668) to (6.7740, 0.0752) to (6.7759, 0.0835) to (6.7778, 0.0916) to (6.7797, 0.0995) to (6.7815, 0.1073) to (6.7832, 0.1150) to (6.7849, 0.1225) to (6.7865, 0.1298) to (6.7881, 0.1371) to (6.7897, 0.1441) to (6.7912, 0.1511) to (6.7923, 0.1565) to (6.7931, 0.1599) to (6.7941, 0.1647) to (6.7955, 0.1713) to (6.7968, 0.1778) to (6.7982, 0.1842) to (6.7994, 0.1905) to (6.8007, 0.1967) to (6.8019, 0.2027) to (6.8031, 0.2087) to (6.8043, 0.2146) to (6.8054, 0.2204) to (6.8065, 0.2261) to (6.8076, 0.2317) to (6.8086, 0.2372) to (6.8097, 0.2426) to (6.8107, 0.2479) to (6.8116, 0.2532) to (6.8126, 0.2583) to (6.8135, 0.2634) to (6.8145, 0.2684) to (6.8153, 0.2734) to (6.8162, 0.2782) to (6.8171, 0.2830) to (6.8179, 0.2878) to (6.8187, 0.2924) to (6.8195, 0.2970) to (6.8200, 0.3001) to (6.8204, 0.3024) to (6.8210, 0.3060) to (6.8218, 0.3103) to (6.8225, 0.3147) to (6.8232, 0.3189) to (6.8239, 0.3231) to (6.8246, 0.3273) to (6.8253, 0.3314) to (6.8259, 0.3354) to (6.8266, 0.3394) to (6.8272, 0.3433) to (6.8337, 0.3821) to (6.8462, 0.4730) to (6.8568, 0.5730) to (6.8638, 0.6603) to (6.8683, 0.7373) to (6.8709, 0.8066) to (6.8726, 0.8875) to (6.8719, 0.9664) to (6.8709, 1.0122) to (6.8696, 1.0527) to (6.8679, 1.0898) to (6.8661, 1.1238) to (6.8641, 1.1552) to (6.8620, 1.1842) to (6.8599, 1.2111) to (6.8577, 1.2362) to (6.8555, 1.2596) to (6.8533, 1.2815) to (6.8513, 1.3003) to (6.8503, 1.3095) to (6.8501, 1.3112) to (6.8500, 1.3122) to (6.8499, 1.3134) to (6.8497, 1.3154) to (6.8494, 1.3174) to (6.8492, 1.3194) to (6.8490, 1.3214) to (6.8487, 1.3235) to (6.8485, 1.3256) to (6.8483, 1.3277) to (6.8480, 1.3297) to (6.8479, 1.3307) to (6.8478, 1.3319) to (6.8475, 1.3341) to (6.8473, 1.3361) to (6.8470, 1.3385) to (6.8467, 1.3407) to (6.8465, 1.3429) to (6.8462, 1.3452) to (6.8459, 1.3474) to (6.8458, 1.3486) to (6.8456, 1.3498) to (6.8453, 1.3522) to (6.8450, 1.3545) to (6.8447, 1.3571) to (6.8445, 1.3592) to (6.8441, 1.3618) to (6.8438, 1.3641) to (6.8437, 1.3654) to (6.8435, 1.3668) to (6.8432, 1.3693) to (6.8429, 1.3719) to (6.8425, 1.3745) to (6.8422, 1.3771) to (6.8418, 1.3797) to (6.8417, 1.3810) to (6.8415, 1.3824) to (6.8411, 1.3851) to (6.8408, 1.3879) to (6.8404, 1.3906) to (6.8400, 1.3934) to (6.8398, 1.3955) to (6.8396, 1.3969) to (6.8393, 1.3991) to (6.8389, 1.4020) to (6.8385, 1.4050) to (6.8380, 1.4079) to (6.8378, 1.4099) to (6.8376, 1.4114) to (6.8372, 1.4140) to (6.8368, 1.4171) to (6.8363, 1.4202) to (6.8359, 1.4229) to (6.8357, 1.4245) to (6.8354, 1.4265) to (6.8349, 1.4298) to (6.8345, 1.4330) to (6.8341, 1.4359) to (6.8338, 1.4375) to (6.8335, 1.4397) to (6.8330, 1.4431) to (6.8325, 1.4466) to (6.8321, 1.4489) to (6.8319, 1.4507) to (6.8314, 1.4536) to (6.8309, 1.4572) to (6.8304, 1.4602) to (6.8301, 1.4620) to (6.8298, 1.4645) to (6.8292, 1.4682) to (6.8287, 1.4714) to (6.8284, 1.4734) to (6.8280, 1.4758) to (6.8274, 1.4797) to (6.8269, 1.4827) to (6.8266, 1.4847) to (6.8261, 1.4876) to (6.8254, 1.4916) to (6.8251, 1.4940) to (6.8247, 1.4960) to (6.8241, 1.4999) to (6.8236, 1.5032) to (6.8232, 1.5053) to (6.8227, 1.5084) to (6.8220, 1.5123) to (6.8217, 1.5145) to (6.8212, 1.5171) to (6.8205, 1.5214) to (6.8201, 1.5237) to (6.8197, 1.5261) to (6.8189, 1.5305) to (6.8185, 1.5328) to (6.8181, 1.5353) to (6.8173, 1.5395) to (6.8169, 1.5419) to (6.8164, 1.5449) to (6.8157, 1.5486) to (6.8153, 1.5510) to (6.8146, 1.5547) to (6.8141, 1.5577) to (6.8136, 1.5601) to (6.8129, 1.5642) to (6.8124, 1.5667) to (6.8118, 1.5700) to (6.8112, 1.5732) to (6.8107, 1.5758) to (6.8100, 1.5796) to (6.8095, 1.5823) to (6.8088, 1.5859) to (6.8083, 1.5887) to (6.8078, 1.5916) to (6.8071, 1.5950) to (6.8066, 1.5978) to (6.8059, 1.6013) to (6.8053, 1.6042) to (6.8047, 1.6075) to (6.8041, 1.6104) to (6.8035, 1.6137) to (6.8029, 1.6167) to (6.8022, 1.6199) to (6.8016, 1.6229) to (6.8010, 1.6261) to (6.8004, 1.6291) to (6.7997, 1.6322) to (6.7991, 1.6353) to (6.7985, 1.6383) to (6.7978, 1.6415) to (6.7972, 1.6444) to (6.7966, 1.6476) to (6.7960, 1.6505) to (6.7953, 1.6538) to (6.7947, 1.6566) to (6.7940, 1.6600) to (6.7934, 1.6627) to (6.7927, 1.6661) to (6.7919, 1.6697) to (6.7912, 1.6732) to (6.7900, 1.6785) to (6.7889, 1.6836) to (6.7878, 1.6887) to (6.7867, 1.6937) to (6.7856, 1.6987) to (6.7845, 1.7035) to (6.7834, 1.7083) to (6.7823, 1.7131) to (6.7813, 1.7178) to (6.7802, 1.7224) to (6.7791, 1.7270) to (6.7781, 1.7315) to (6.7770, 1.7360) to (6.7760, 1.7404) to (6.7750, 1.7448) to (6.7739, 1.7492) to (6.7729, 1.7535) to (6.7719, 1.7578) to (6.7708, 1.7621) to (6.7698, 1.7663) to (6.7688, 1.7705) to (6.7678, 1.7747) to (6.7667, 1.7789) to (6.7657, 1.7830) to (6.7647, 1.7872) to (6.7636, 1.7913) to (6.7626, 1.7954) to (6.7616, 1.7995) to (6.7605, 1.8036) to (6.7595, 1.8077) to (6.7584, 1.8118) to (6.7574, 1.8158) to (6.7563, 1.8199) to (6.7553, 1.8240) to (6.7542, 1.8281) to (6.7531, 1.8322) to (6.7520, 1.8363) to (6.7510, 1.8404) to (6.7499, 1.8445) to (6.7487, 1.8487) to (6.7476, 1.8528) to (6.7465, 1.8570) to (6.7454, 1.8612) to (6.7442, 1.8654) to (6.7430, 1.8697) to (6.7414, 1.8756) to (6.6954, 2.0345) to (6.6181, 2.2741) to (6.5391, 2.4923) to (6.4583, 2.6946) to (6.3757, 2.8839) to (6.2911, 3.0628) to (6.2046, 3.2329) to (6.1161, 3.3954) to (6.0255, 3.5514) to (5.9329, 3.7015) to (5.8380, 3.8463) to (5.7410, 3.9863) to (5.6418, 4.1219) to (5.5401, 4.2534) to (5.4363, 4.3810) to (5.3299, 4.5050) to (5.2211, 4.6255) to (5.1099, 4.7425) to (4.9961, 4.8563) to (4.8799, 4.9668) to (4.7609, 5.0742) to (4.6394, 5.1784) to (4.5153, 5.2795) to (4.3885, 5.3774) to (4.2590, 5.4720) to (4.1269, 5.5635) to (3.9921, 5.6516) to (3.8547, 5.7364) to (3.7146, 5.8177) to (3.5720, 5.8955) to (3.4268, 5.9697) to (3.2791, 6.0402) to (3.1290, 6.1069) to (2.9765, 6.1696) to (2.8217, 6.2283) to (2.6648, 6.2829) to (2.5059, 6.3332) to (2.3451, 6.3791) to (2.1824, 6.4206) to (2.0182, 6.4574) to (1.8526, 6.4896) to (1.6857, 6.5170) to (1.5177, 6.5396) to (1.3489, 6.5572) to (1.1795, 6.5699) to (1.0097, 6.5775) to (0.8398, 6.5800) to (0.6699, 6.5775) to (0.5005, 6.5699) to (0.3316, 6.5572) to (0.1636, 6.5394) to (0.0263, 6.5211) to (-0.2031, 6.4827) to (-0.2150, 6.4804) to (-0.2967, 6.4641) to (-0.3842, 6.4453) to (-0.4750, 6.4241) to (-0.5557, 6.4040) to (-0.6472, 6.3795) to (-0.7265, 6.3570) to (-0.8132, 6.3308) to (-0.8912, 6.3060) to (-0.9730, 6.2784) to (-1.0496, 6.2514) to (-1.1269, 6.2227) to (-1.2020, 6.1936) to (-1.2749, 6.1641) to (-1.3485, 6.1331) to (-1.4171, 6.1030) to (-1.4892, 6.0701) to (-1.5537, 6.0395) to (-1.6243, 6.0049) to (-1.6849, 5.9740) to (-1.7540, 5.9378) to (-1.8110, 5.9068) to (-1.8663, 5.8760) to (-1.9320, 5.8381) to (-1.9833, 5.8077) to (-2.0481, 5.7681) to (-2.0962, 5.7379) to (-2.1595, 5.6970) to (-2.2046, 5.6669) to (-2.2527, 5.6343) to (-2.3088, 5.5952) to (-2.3495, 5.5661) to (-2.4089, 5.5226) to (-2.4470, 5.4939) to (-2.4894, 5.4614) to (-2.5406, 5.4212) to (-2.5749, 5.3937) to (-2.6266, 5.3513) to (-2.6628, 5.3209) to (-2.6937, 5.2945) to (-2.7473, 5.2476) to (-2.7763, 5.2217) to (-2.8065, 5.1943) to (-2.8558, 5.1486) to (-2.8819, 5.1239) to (-2.9117, 5.0953) to (-2.9569, 5.0510) to (-2.9805, 5.0273) to (-3.0068, 5.0007) to (-3.0509, 4.9550) to (-3.0726, 4.9321) to (-3.0932, 4.9100) to (-3.1330, 4.8668) to (-3.1588, 4.8381) to (-3.1775, 4.8171) to (-3.2077, 4.7826) to (-3.2396, 4.7454) to (-3.2566, 4.7253) to (-3.2759, 4.7022) to (-3.3078, 4.6635) to (-3.3310, 4.6347) to (-3.3459, 4.6159) to (-3.3675, 4.5885) to (-3.3955, 4.5523) to (-3.4146, 4.5272) to (-3.4278, 4.5097) to (-3.4481, 4.4824) to (-3.4728, 4.4485) to (-3.4914, 4.4226) to (-3.5030, 4.4063) to (-3.5133, 4.3918) to (-3.5248, 4.3753) to (-3.5360, 4.3590) to (-3.5415, 4.3509) to (-3.5469, 4.3429) to (-3.5577, 4.3270) to (-3.5681, 4.3113) to (-3.5771, 4.2977) to (-3.5821, 4.2900) to (-3.5883, 4.2805) to (-3.5980, 4.2654) to (-3.6075, 4.2504) to (-3.6163, 4.2365) to (-3.6208, 4.2292) to (-3.6258, 4.2211) to (-3.6347, 4.2067) to (-3.6434, 4.1925) to (-3.6518, 4.1785) to (-3.6579, 4.1684) to (-3.6620, 4.1615) to (-3.6682, 4.1509) to (-3.6761, 4.1374) to (-3.6838, 4.1241) to (-3.6914, 4.1109) to (-3.6971, 4.1009) to (-3.7007, 4.0944) to (-3.7060, 4.0850) to (-3.7131, 4.0723) to (-3.7200, 4.0597) to (-3.7268, 4.0474) to (-3.7334, 4.0351) to (-3.7374, 4.0278) to (-3.7406, 4.0217) to (-3.7462, 4.0111) to (-3.7524, 3.9993) to (-3.7585, 3.9877) to (-3.7645, 3.9761) to (-3.7693, 3.9668) to (-3.7721, 3.9612) to (-3.7743, 3.9570) to (-3.7760, 3.9535) to (-3.7778, 3.9501) to (-3.7792, 3.9472) to (-3.7817, 3.9423) to (-3.7841, 3.9375) to (-3.7861, 3.9335) to (-3.7888, 3.9280) to (-3.7909, 3.9239) to (-3.7935, 3.9185) to (-3.7955, 3.9145) to (-3.7978, 3.9097) to (-3.8001, 3.9051) to (-3.8020, 3.9012) to (-3.8045, 3.8959) to (-3.8064, 3.8920) to (-3.8089, 3.8868) to (-3.8108, 3.8829) to (-3.8130, 3.8783) to (-3.8149, 3.8744) to (-3.8151, 3.8739) to (-3.8169, 3.8701) to (-3.8193, 3.8650) to (-3.8211, 3.8612) to (-3.8235, 3.8562) to (-3.8252, 3.8524) to (-3.8274, 3.8478) to (-3.8293, 3.8437) to (-3.8310, 3.8400) to (-3.8333, 3.8351) to (-3.8349, 3.8315) to (-3.8371, 3.8266) to (-3.8388, 3.8230) to (-3.8409, 3.8185) to (-3.8426, 3.8146) to (-3.8442, 3.8110) to (-3.8464, 3.8063) to (-3.8480, 3.8028) to (-3.8500, 3.7981) to (-3.8516, 3.7946) to (-3.8521, 3.7934) to (-3.8537, 3.7899) to (-3.8552, 3.7865) to (-3.8567, 3.7830) to (-3.8587, 3.7785) to (-3.8603, 3.7751) to (-3.8622, 3.7706) to (-3.8637, 3.7671) to (-3.8656, 3.7628) to (-3.8671, 3.7593) to (-3.8685, 3.7560) to (-3.8704, 3.7516) to (-3.8719, 3.7483) to (-3.8737, 3.7439) to (-3.8751, 3.7407) to (-3.8769, 3.7364) to (-3.8784, 3.7330) to (-3.8797, 3.7299) to (-3.8815, 3.7256) to (-3.8828, 3.7224) to (-3.8846, 3.7182) to (-3.8859, 3.7150) to (-3.8875, 3.7111) to (-3.8888, 3.7080) to (-3.8890, 3.7077) to (-3.8903, 3.7046) to (-3.8920, 3.7005) to (-3.8932, 3.6974) to (-3.8949, 3.6933) to (-3.8961, 3.6903) to (-3.8978, 3.6862) to (-3.8990, 3.6832) to (-3.9003, 3.6801) to (-3.9018, 3.6762) to (-3.9030, 3.6732) to (-3.9046, 3.6693) to (-3.9058, 3.6663) to (-3.9074, 3.6624) to (-3.9085, 3.6595) to (-3.9098, 3.6564) to (-3.9112, 3.6527) to (-3.9124, 3.6498) to (-3.9139, 3.6460) to (-3.9150, 3.6431) to (-3.9165, 3.6393) to (-3.9176, 3.6365) to (-3.9188, 3.6335) to (-3.9201, 3.6299) to (-3.9212, 3.6271) to (-3.9226, 3.6234) to (-3.9237, 3.6207) to (-3.9242, 3.6194) to (-3.9251, 3.6170) to (-3.9261, 3.6142) to (-3.9273, 3.6113) to (-3.9286, 3.6079) to (-3.9296, 3.6052) to (-3.9310, 3.6016) to (-3.9320, 3.5989) to (-3.9333, 3.5954) to (-3.9343, 3.5927) to (-3.9354, 3.5898) to (-3.9366, 3.5866) to (-3.9376, 3.5839) to (-3.9388, 3.5805) to (-3.9398, 3.5778) to (-3.9411, 3.5744) to (-3.9420, 3.5718) to (-3.9431, 3.5689) to (-3.9442, 3.5659) to (-3.9451, 3.5633) to (-3.9463, 3.5600) to (-3.9473, 3.5574) to (-3.9485, 3.5541) to (-3.9494, 3.5516) to (-3.9504, 3.5488) to (-3.9515, 3.5458) to (-3.9523, 3.5434) to (-3.9535, 3.5401) to (-3.9544, 3.5377) to (-3.9555, 3.5344) to (-3.9564, 3.5320) to (-3.9573, 3.5293) to (-3.9582, 3.5269) to (-3.9584, 3.5264) to (-3.9592, 3.5240) to (-3.9603, 3.5208) to (-3.9611, 3.5185) to (-3.9622, 3.5153) to (-3.9630, 3.5130) to (-3.9640, 3.5102) to (-3.9649, 3.5076) to (-3.9657, 3.5053) to (-3.9668, 3.5021) to (-3.9676, 3.4999) to (-3.9686, 3.4968) to (-3.9694, 3.4945) to (-3.9703, 3.4918) to (-3.9712, 3.4893) to (-3.9720, 3.4870) to (-3.9730, 3.4840) to (-3.9737, 3.4818) to (-3.9747, 3.4788) to (-3.9755, 3.4766) to (-3.9764, 3.4739) to (-3.9772, 3.4715) to (-3.9779, 3.4693) to (-3.9789, 3.4664) to (-3.9796, 3.4642) to (-3.9805, 3.4614) to (-3.9813, 3.4592) to (-3.9821, 3.4565) to (-3.9829, 3.4543) to (-3.9836, 3.4521) to (-3.9845, 3.4493) to (-3.9852, 3.4472) to (-3.9861, 3.4444) to (-3.9868, 3.4423) to (-3.9876, 3.4397) to (-3.9883, 3.4375) to (-3.9890, 3.4354) to (-3.9899, 3.4327) to (-3.9904, 3.4312) to (-3.9908, 3.4300) to (-3.9914, 3.4280) to (-3.9921, 3.4259) to (-3.9929, 3.4233) to (-3.9935, 3.4212) to (-3.9942, 3.4192) to (-3.9950, 3.4166) to (-3.9956, 3.4146) to (-3.9965, 3.4119) to (-3.9971, 3.4100) to (-3.9979, 3.4074) to (-3.9985, 3.4054) to (-3.9991, 3.4034) to (-3.9999, 3.4009) to (-4.0005, 3.3989) to (-4.0013, 3.3964) to (-4.0019, 3.3945) to (-4.0027, 3.3919) to (-4.0041, 3.3875) to (-4.0056, 3.3825) to (-4.0071, 3.3776) to (-4.0086, 3.3726) to (-4.0100, 3.3678) to (-4.0115, 3.3630) to (-4.0129, 3.3582) to (-4.0143, 3.3534) to (-4.0157, 3.3487) to (-4.0171, 3.3441) to (-4.0184, 3.3395) to (-4.0197, 3.3349) to (-4.0208, 3.3313) to (-4.0214, 3.3291) to (-4.0223, 3.3259) to (-4.0236, 3.3214) to (-4.0249, 3.3170) to (-4.0261, 3.3126) to (-4.0273, 3.3083) to (-4.0285, 3.3040) to (-4.0297, 3.2997) to (-4.0309, 3.2955) to (-4.0321, 3.2913) to (-4.0331, 3.2874) to (-4.0343, 3.2831) to (-4.0354, 3.2790) to (-4.0365, 3.2749) to (-4.0376, 3.2709) to (-4.0387, 3.2669) to (-4.0398, 3.2630) to (-4.0408, 3.2591) to (-4.0418, 3.2552) to (-4.0429, 3.2513) to (-4.0439, 3.2475) to (-4.0448, 3.2437) to (-4.0458, 3.2399) to (-4.0468, 3.2362) to (-4.0478, 3.2325) to (-4.0487, 3.2288) to (-4.0493, 3.2263) to (-4.0498, 3.2245) to (-4.0506, 3.2216) to (-4.0515, 3.2180) to (-4.0524, 3.2144) to (-4.0532, 3.2109) to (-4.0541, 3.2074) to (-4.0550, 3.2039) to (-4.0558, 3.2005) to (-4.0567, 3.1971) to (-4.0575, 3.1937) to (-4.0584, 3.1903) to (-4.0675, 3.1528) to (-4.0879, 3.0607) to (-4.1095, 2.9464) to (-4.1277, 2.8283) to (-4.1424, 2.7066) to (-4.1530, 2.5815) to (-4.1593, 2.4529) to (-4.1609, 2.3228) to (-4.1577, 2.1891) to (-4.1492, 2.0538) to (-4.1354, 1.9169) to (-4.1160, 1.7791) to (-4.0910, 1.6409) to (-4.0603, 1.5029) to (-4.0239, 1.3656) to (-3.9820, 1.2296) to (-3.9348, 1.0955) to (-3.8824, 0.9638) to (-3.8251, 0.8351) to (-3.7688, 0.7218) to (-3.7386, 0.6677) to (-3.7328, 0.6569) to (-3.7295, 0.6508) to (-3.7253, 0.6433) to (-3.7185, 0.6309) to (-3.7115, 0.6183) to (-3.7044, 0.6056) to (-3.6971, 0.5927) to (-3.6896, 0.5796) to (-3.6819, 0.5664) to (-3.6741, 0.5530) to (-3.6663, 0.5397) to (-3.6622, 0.5330) to (-3.6580, 0.5257) to (-3.6496, 0.5118) to (-3.6410, 0.4978) to (-3.6323, 0.4835) to (-3.6233, 0.4691) to (-3.6141, 0.4545) to (-3.6047, 0.4397) to (-3.5955, 0.4254) to (-3.5906, 0.4180) to (-3.5852, 0.4096) to (-3.5752, 0.3942) to (-3.5648, 0.3787) to (-3.5542, 0.3629) to (-3.5434, 0.3470) to (-3.5323, 0.3308) to (-3.5217, 0.3157) to (-3.5159, 0.3076) to (-3.5092, 0.2979) to (-3.4973, 0.2812) to (-3.4850, 0.2642) to (-3.4725, 0.2471) to (-3.4596, 0.2297) to (-3.4465, 0.2121) to (-3.4397, 0.2036) to (-3.4329, 0.1943) to (-3.4190, 0.1762) to (-3.4048, 0.1580) to (-3.3902, 0.1395) to (-3.3752, 0.1208) to (-3.3642, 0.1077) to (-3.3564, 0.0981) to (-3.3441, 0.0826) to (-3.3279, 0.0630) to (-3.3114, 0.0429) to (-3.2943, 0.0214) to (-3.2828, 0.0111) to (-3.2767,0.0000) to (-3.2667,0.0000) to (-3.2626,0.0000) to (-3.2526,0.0000) to (-3.2444,0.0000) to (-3.2344,0.0000) to (-3.2264,0.0000) to (-3.2222,0.0000) to (-3.2122,0.0000) to (-3.2044,0.0000) to (-3.1944,0.0000) to (-3.1868,0.0000) to (-3.1818,0.0000) to (-3.1718,0.0000) to (-3.1644,0.0000) to (-3.1544,0.0000) to (-3.1472,0.0000) to (-3.1414,0.0000) to (-3.1314,0.0000) to (-3.1244,0.0000) to (-3.1144,0.0000) to (-3.1120,0.0000) to (-3.1020,0.0000) to (-3.1010,0.0000) to (-3.0910,0.0000) to (-3.0844,0.0000) to (-3.0744,0.0000) to (-3.0680,0.0000) to (-3.0606,0.0000) to (-3.0444, 0.0000) to (-3.0283, 0.0000) to (-3.0202, 0.0000) to (-3.0044, 0.0000) to (-2.9887, 0.0000) to (-2.9798, 0.0000) to (-2.9644, 0.0000) to (-2.9509, 0.0000) to (-2.9394, 0.0000) to (-2.9243, 0.0000) to (-2.9094, 0.0000) to (-2.8990, 0.0000) to (-2.8843, 0.0000) to (-2.8697, 0.0000) to (-2.8586, 0.0000) to (-2.8442, 0.0000) to (-2.8300, 0.0000) to (-2.8182, 0.0000) to (-2.8071, 0.0101) to (-2.7936, 0.0267) to (-2.7767, 0.0482) to (-2.7623, 0.0665) to (-2.7534, 0.0773) to (-2.7414, 0.0903) to (-2.7229, 0.1116) to (-2.7065, 0.1304) to (-2.6968, 0.1414) to (-2.6841, 0.1547) to (-2.6638, 0.1767) to (-2.6478, 0.1941) to (-2.6371, 0.2053) to (-2.6212, 0.2213) to (-2.5989, 0.2439) to (-2.5859, 0.2575) to (-2.5742, 0.2686) to (-2.5522, 0.2900) to (-2.5330, 0.3085) to (-2.5206, 0.3203) to (-2.5024, 0.3369) to (-2.4786, 0.3586) to (-2.4654, 0.3708) to (-2.4495, 0.3845) to (-2.4226, 0.4079) to (-2.4085, 0.4203) to (-2.3931, 0.4329) to (-2.3649, 0.4563) to (-2.3499, 0.4688) to (-2.3332, 0.4818) to (-2.3055, 0.5038) to (-2.2895, 0.5163) to (-2.2696, 0.5312) to (-2.2443, 0.5502) to (-2.2275, 0.5626) to (-2.2020, 0.5807) to (-2.1814, 0.5955) to (-2.1636, 0.6078) to (-2.1352, 0.6272) to (-2.1167, 0.6397) to (-2.0929, 0.6551) to (-2.0697, 0.6703) to (-2.0502, 0.6824) to (-2.0224, 0.6997) to (-2.0024, 0.7120) to (-1.9750, 0.7281) to (-1.9543, 0.7404) to (-1.9323, 0.7527) to (-1.9060, 0.7677) to (-1.8843, 0.7795) to (-1.8576, 0.7940) to (-1.8352, 0.8057) to (-1.8089, 0.8193) to (-1.7860, 0.8309) to (-1.7601, 0.8436) to (-1.7365, 0.8550) to (-1.7110, 0.8669) to (-1.6869, 0.8782) to (-1.6618, 0.8893) to (-1.6370, 0.9003) to (-1.6123, 0.9108) to (-1.5870, 0.9215) to (-1.4274, 0.9729) to (-1.0454, 0.9979) to (-0.5404, 0.7895) to (-0.3900, 0.6494) to (-0.3867, 0.6456) to (-0.3828, 0.6414) to (-0.3795, 0.6377) to (-0.3754, 0.6333) to (-0.3720, 0.6297) to (-0.3677, 0.6251) to (-0.3631, 0.6204) to (-0.3584, 0.6157) to (-0.3512, 0.6086) to (-0.3439, 0.6016) to (-0.3365, 0.5946) to (-0.3289, 0.5877) to (-0.3211, 0.5807) to (-0.3130, 0.5738) to (-0.3048, 0.5668) to (-0.2962, 0.5597) to (-0.2873, 0.5525) to (-0.2777, 0.5449) to (-0.2674, 0.5368) to (-0.2556, 0.5278) to (-0.2413, 0.5169) to (-0.2218, 0.5018) to (-0.1894, 0.4754) to (-0.1152, 0.4027) to (0.0088, 0.1901) to (0.0338, 0.0897) to (0.0353, 0.0802) to (0.0356, 0.0778) to (0.0360, 0.0754) to (0.0363, 0.0730) to (0.0367, 0.0706) to (0.0371, 0.0682) to (0.0374, 0.0658) to (0.0378, 0.0634) to (0.0381, 0.0610) to (0.0385, 0.0586) to (0.0389, 0.0563) to (0.0392, 0.0539) to (0.0396, 0.0515) to (0.0400, 0.0492) to (0.0404, 0.0468) to (0.0407, 0.0444) to (0.0411, 0.0420) to (0.0415, 0.0396) to (0.0419, 0.0372) to (0.0423, 0.0348) to (0.0427, 0.0324) to (0.0431, 0.0299) to (0.0435, 0.0275) to (0.0439, 0.0250) to (0.0443, 0.0225) to (0.0447, 0.0200) to (0.0451, 0.0174) to (0.0455, 0.0148) to (0.0460, 0.0122) to (0.0464, 0.0094) to (0.0468, 0.0065) to cycle; \end{scope}
